Q4EDA: A Novel Strategy for Textual Information Retrieval Based on User Interactions with Visual Representations of Time Series

Knowing how to construct text-based Search Queries (SQs) for use in Search Engines (SEs) such as Google or Wikipedia has become a fundamental skill. Though much data are available through such SEs, most structured datasets live outside their scope. Visualization tools aid in this limitation, but no such tools come close to the sheer amount of information available through general-purpose SEs. To fill this gap, this paper presents Q4EDA, a novel framework that converts users' visual selection queries executed on top of time series visual representations, providing valid and stable SQs to be used in general-purpose SEs and suggestions of related information. The usefulness of Q4EDA is presented and validated by users through an application linking a Gapminder's line-chart replica with a SE populated with Wikipedia documents, showing how Q4EDA supports and enhances exploratory analysis of United Nations world indicators. Despite some limitations, Q4EDA is unique in its proposal and represents a real advance towards providing solutions for querying textual information based on user interactions with visual representations.

==> MDPIDefinitions/journalnames.tex <==
%%Updated on 20 April 2022
%,% Website Name,%,%,% Website Name,%%,% Full Name,%%,% Short Name,%%,% DOI abbr,%%,% ISSN,% \continuouspages
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{acoustics}{\gdef\@journal{acoustics}\gdef\@journalfull{Acoustics}\gdef\@journalshort{Acoustics}\gdef\@doiabbr{acoustics}\gdef\@ISSN{2624-599X}\gdef\@continuouspages{yes}}
\DeclareOption{actuators}{\gdef\@journal{actuators}\gdef\@journalfull{Actuators}\gdef\@journalshort{Actuators}\gdef\@doiabbr{act}\gdef\@ISSN{2076-0825}}
\DeclareOption{addictions}{\gdef\@journal{addictions}\gdef\@journalfull{Addictions}\gdef\@journalshort{Addictions}\gdef\@doiabbr{}\gdef\@ISSN{0006-0006}}
\DeclareOption{admsci}{\gdef\@journal{admsci}\gdef\@journalfull{Administrative Sciences}\gdef\@journalshort{Adm. Sci.}\gdef\@doiabbr{admsci}\gdef\@ISSN{2076-3387}}
\DeclareOption{adolescents}{\gdef\@journal{adolescents}\gdef\@journalfull{Adolescents}\gdef\@journalshort{Adolescents}\gdef\@doiabbr{adolescents}\gdef\@ISSN{2673-7051}\gdef\@continuouspages{yes}}
\DeclareOption{aerospace}{\gdef\@journal{aerospace}\gdef\@journalfull{Aerospace}\gdef\@journalshort{Aerospace}\gdef\@doiabbr{aerospace}\gdef\@ISSN{2226-4310}}
\DeclareOption{agriculture}{\gdef\@journal{agriculture}\gdef\@journalfull{Agriculture}\gdef\@journalshort{Agriculture}\gdef\@doiabbr{agriculture}\gdef\@ISSN{2077-0472}}
\DeclareOption{agriengineering}{\gdef\@journal{agriengineering}\gdef\@journalfull{AgriEngineering}\gdef\@journalshort{AgriEngineering}\gdef\@doiabbr{agriengineering}\gdef\@ISSN{2624-7402}\gdef\@continuouspages{yes}}
\DeclareOption{agrochemicals}{\gdef\@journal{agrochemicals}\gdef\@journalfull{Agrochemicals}\gdef\@journalshort{Agrochemicals}\gdef\@doiabbr{agrochemicals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{agronomy}{\gdef\@journal{agronomy}\gdef\@journalfull{Agronomy}\gdef\@journalshort{Agronomy}\gdef\@doiabbr{agronomy}\gdef\@ISSN{2073-4395}}
\DeclareOption{ai}{\gdef\@journal{ai}\gdef\@journalfull{AI}\gdef\@journalshort{AI}\gdef\@doiabbr{ai}\gdef\@ISSN{2673-2688}\gdef\@continuouspages{yes}}
\DeclareOption{air}{\gdef\@journal{air}\gdef\@journalfull{Air}\gdef\@journalshort{Air}\gdef\@doiabbr{air}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{algorithms}{\gdef\@journal{algorithms}\gdef\@journalfull{Algorithms}\gdef\@journalshort{Algorithms}\gdef\@doiabbr{a}\gdef\@ISSN{1999-4893}}
\DeclareOption{allergies}{\gdef\@journal{allergies}\gdef\@journalfull{Allergies}\gdef\@journalshort{Allergies}\gdef\@doiabbr{allergies}\gdef\@ISSN{2313-5786}}
\DeclareOption{alloys}{\gdef\@journal{alloys}\gdef\@journalfull{Alloys}\gdef\@journalshort{Alloys}\gdef\@doiabbr{alloys}\gdef\@ISSN{2674-063X}\gdef\@continuouspages{yes}}
\DeclareOption{analytica}{\gdef\@journal{analytica}\gdef\@journalfull{Analytica}\gdef\@journalshort{Analytica}\gdef\@doiabbr{analytica}\gdef\@ISSN{2673-4532}\gdef\@continuouspages{yes}}
\DeclareOption{analytics}{\gdef\@journal{analytics}\gdef\@journalfull{Analytics}\gdef\@journalshort{Analytics}\gdef\@doiabbr{analytics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{anatomia}{\gdef\@journal{anatomia}\gdef\@journalfull{Anatomia}\gdef\@journalshort{Anatomia}\gdef\@doiabbr{anatomia}\gdef\@ISSN{2813-0545}\gdef\@continuouspages{yes}}
\DeclareOption{animals}{\gdef\@journal{animals}\gdef\@journalfull{Animals}\gdef\@journalshort{Animals}\gdef\@doiabbr{ani}\gdef\@ISSN{2076-2615}}
\DeclareOption{antibiotics}{\gdef\@journal{antibiotics}\gdef\@journalfull{Antibiotics}\gdef\@journalshort{Antibiotics}\gdef\@doiabbr{antibiotics}\gdef\@ISSN{2079-6382}}
\DeclareOption{antibodies}{\gdef\@journal{antibodies}\gdef\@journalfull{Antibodies}\gdef\@journalshort{Antibodies}\gdef\@doiabbr{antib}\gdef\@ISSN{2073-4468}}
\DeclareOption{antioxidants}{\gdef\@journal{antioxidants}\gdef\@journalfull{Antioxidants}\gdef\@journalshort{Antioxidants}\gdef\@doiabbr{antiox}\gdef\@ISSN{2076-3921}}
\DeclareOption{applbiosci}{\gdef\@journal{applbiosci}\gdef\@journalfull{Applied Biosciences}\gdef\@journalshort{Appl. Biosci.}\gdef\@doiabbr{applbiosci}\gdef\@ISSN{2813-0464}\gdef\@continuouspages{yes}}
\DeclareOption{appliedchem}{\gdef\@journal{appliedchem}\gdef\@journalfull{AppliedChem}\gdef\@journalshort{AppliedChem}\gdef\@doiabbr{appliedchem}\gdef\@ISSN{2673-9623}\gdef\@continuouspages{yes}}
\DeclareOption{appliedmath}{\gdef\@journal{appliedmath}\gdef\@journalfull{AppliedMath}\gdef\@journalshort{AppliedMath}\gdef\@doiabbr{appliedmath}\gdef\@ISSN{2673-9909}\gdef\@continuouspages{yes}}
\DeclareOption{applmech}{\gdef\@journal{applmech}\gdef\@journalfull{Applied Mechanics}\gdef\@journalshort{Appl. Mech.}\gdef\@doiabbr{applmech}\gdef\@ISSN{2673-3161}\gdef\@continuouspages{yes}}
\DeclareOption{applmicrobiol}{\gdef\@journal{applmicrobiol}\gdef\@journalfull{Applied Microbiology}\gdef\@journalshort{Appl. Microbiol.}\gdef\@doiabbr{applmicrobiol}\gdef\@ISSN{2673-8007}\gdef\@continuouspages{yes}}
\DeclareOption{applnano}{\gdef\@journal{applnano}\gdef\@journalfull{Applied Nano}\gdef\@journalshort{Appl. Nano}\gdef\@doiabbr{applnano}\gdef\@ISSN{2673-3501}\gdef\@continuouspages{yes}}
\DeclareOption{applsci}{\gdef\@journal{applsci}\gdef\@journalfull{Applied Sciences}\gdef\@journalshort{Appl. Sci.}\gdef\@doiabbr{app}\gdef\@ISSN{2076-3417}}
\DeclareOption{aquacj}{\gdef\@journal{aquacj}\gdef\@journalfull{Aquaculture Journal}\gdef\@journalshort{Aquac. J.}\gdef\@doiabbr{aj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{architecture}{\gdef\@journal{architecture}\gdef\@journalfull{Architecture}\gdef\@journalshort{Architecture}\gdef\@doiabbr{architecture}\gdef\@ISSN{2673-8945}\gdef\@continuouspages{yes}}
\DeclareOption{arts}{\gdef\@journal{arts}\gdef\@journalfull{Arts}\gdef\@journalshort{Arts}\gdef\@doiabbr{arts}\gdef\@ISSN{2076-0752}}
\DeclareOption{asc}{\gdef\@journal{asc}\gdef\@journalfull{Automatic Systems and Control}\gdef\@journalshort{Autom. Syst. Control}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{asi}{\gdef\@journal{asi}\gdef\@journalfull{Applied System Innovation}\gdef\@journalshort{Appl. Syst. Innov.}\gdef\@doiabbr{asi}\gdef\@ISSN{2571-5577}}
\DeclareOption{astronomy}{\gdef\@journal{astronomy}\gdef\@journalfull{Astronomy}\gdef\@journalshort{Astronomy}\gdef\@doiabbr{astronomy}\gdef\@ISSN{2674-0346}\gdef\@continuouspages{yes}}
\DeclareOption{atmosphere}{\gdef\@journal{atmosphere}\gdef\@journalfull{Atmosphere}\gdef\@journalshort{Atmosphere}\gdef\@doiabbr{atmos}\gdef\@ISSN{2073-4433}}
\DeclareOption{atoms}{\gdef\@journal{atoms}\gdef\@journalfull{Atoms}\gdef\@journalshort{Atoms}\gdef\@doiabbr{atoms}\gdef\@ISSN{2218-2004}}
\DeclareOption{audiolres}{\gdef\@journal{audiolres}\gdef\@journalfull{Audiology Research}\gdef\@journalshort{Audiol. Res.}\gdef\@doiabbr{audiolres}\gdef\@ISSN{2039-4349}\gdef\@continuouspages{yes}}
\DeclareOption{automation}{\gdef\@journal{automation}\gdef\@journalfull{Automation}\gdef\@journalshort{Automation}\gdef\@doiabbr{automation}\gdef\@ISSN{2673-4052}\gdef\@continuouspages{yes}}
\DeclareOption{axioms}{\gdef\@journal{axioms}\gdef\@journalfull{Axioms}\gdef\@journalshort{Axioms}\gdef\@doiabbr{axioms}\gdef\@ISSN{2075-1680}}
\DeclareOption{bacteria}{\gdef\@journal{bacteria}\gdef\@journalfull{Bacteria}\gdef\@journalshort{Bacteria}\gdef\@doiabbr{bacteria}\gdef\@ISSN{2674-1334}\gdef\@continuouspages{yes}}
\DeclareOption{batteries}{\gdef\@journal{batteries}\gdef\@journalfull{Batteries}\gdef\@journalshort{Batteries}\gdef\@doiabbr{batteries}\gdef\@ISSN{2313-0105}}
\DeclareOption{bdcc}{\gdef\@journal{bdcc}\gdef\@journalfull{Big Data and Cognitive Computing}\gdef\@journalshort{Big Data Cogn. Comput.}\gdef\@doiabbr{bdcc}\gdef\@ISSN{2504-2289}}
\DeclareOption{behavsci}{\gdef\@journal{behavsci}\gdef\@journalfull{Behavioral Sciences}\gdef\@journalshort{Behav. Sci.}\gdef\@doiabbr{bs}\gdef\@ISSN{2076-328X}}
\DeclareOption{beverages}{\gdef\@journal{beverages}\gdef\@journalfull{Beverages}\gdef\@journalshort{Beverages}\gdef\@doiabbr{beverages}\gdef\@ISSN{2306-5710}}
\DeclareOption{biochem}{\gdef\@journal{biochem}\gdef\@journalfull{BioChem}\gdef\@journalshort{BioChem}\gdef\@doiabbr{biochem}\gdef\@ISSN{2673-6411}\gdef\@continuouspages{yes}}
\DeclareOption{bioengineering}{\gdef\@journal{bioengineering}\gdef\@journalfull{Bioengineering}\gdef\@journalshort{Bioengineering}\gdef\@doiabbr{bioengineering}\gdef\@ISSN{2306-5354}}
\DeclareOption{biologics}{\gdef\@journal{biologics}\gdef\@journalfull{Biologics}\gdef\@journalshort{Biologics}\gdef\@doiabbr{biologics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biology}{\gdef\@journal{biology}\gdef\@journalfull{Biology}\gdef\@journalshort{Biology}\gdef\@doiabbr{biology}\gdef\@ISSN{2079-7737}}
\DeclareOption{biomass}{\gdef\@journal{biomass}\gdef\@journalfull{Biomass}\gdef\@journalshort{Biomass}\gdef\@doiabbr{biomass}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomechanics}{\gdef\@journal{biomechanics}\gdef\@journalfull{Biomechanics}\gdef\@journalshort{Biomechanics}\gdef\@doiabbr{biomechanics}\gdef\@ISSN{2673-7078}\gdef\@continuouspages{yes}}
\DeclareOption{biomed}{\gdef\@journal{biomed}\gdef\@journalfull{BioMed}\gdef\@journalshort{BioMed}\gdef\@doiabbr{biomed}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomedicines}{\gdef\@journal{biomedicines}\gdef\@journalfull{Biomedicines}\gdef\@journalshort{Biomedicines}\gdef\@doiabbr{biomedicines}\gdef\@ISSN{2227-9059}}
\DeclareOption{biomedinformatics}{\gdef\@journal{biomedinformatics}\gdef\@journalfull{Biomedinformatics}\gdef\@journalshort{Biomedinformatics}\gdef\@doiabbr{biomedinformatics}\gdef\@ISSN{2673-7426}\gdef\@continuouspages{yes}}
\DeclareOption{biomimetics}{\gdef\@journal{biomimetics}\gdef\@journalfull{Biomimetics}\gdef\@journalshort{Biomimetics}\gdef\@doiabbr{biomimetics}\gdef\@ISSN{2313-7673}}
\DeclareOption{biomolecules}{\gdef\@journal{biomolecules}\gdef\@journalfull{Biomolecules}\gdef\@journalshort{Biomolecules}\gdef\@doiabbr{biom}\gdef\@ISSN{2218-273X}}
\DeclareOption{biophysica}{\gdef\@journal{biophysica}\gdef\@journalfull{Biophysica}\gdef\@journalshort{Biophysica}\gdef\@doiabbr{biophysica}\gdef\@ISSN{2673-4125}\gdef\@continuouspages{yes}}
\DeclareOption{biosensors}{\gdef\@journal{biosensors}\gdef\@journalfull{Biosensors}\gdef\@journalshort{Biosensors}\gdef\@doiabbr{bios}\gdef\@ISSN{2079-6374}}
\DeclareOption{biotech}{\gdef\@journal{biotech}\gdef\@journalfull{BioTech}\gdef\@journalshort{BioTech}\gdef\@doiabbr{biotech}\gdef\@ISSN{2673-6284}}
\DeclareOption{birds}{\gdef\@journal{birds}\gdef\@journalfull{Birds}\gdef\@journalshort{Birds}\gdef\@doiabbr{birds}\gdef\@ISSN{2673-6004}\gdef\@continuouspages{yes}}
\DeclareOption{bloods}{\gdef\@journal{bloods}\gdef\@journalfull{Bloods}\gdef\@journalshort{Bloods}\gdef\@doiabbr{bloods}\gdef\@ISSN{2673-415X}}
\DeclareOption{blsf}{\gdef\@journal{blsf}\gdef\@journalfull{Biology and Life Sciences Forum}\gdef\@journalshort{Biol. Life Sci. Forum}\gdef\@doiabbr{blsf	}\gdef\@ISSN{2673-9976}}
\DeclareOption{brainsci}{\gdef\@journal{brainsci}\gdef\@journalfull{Brain Sciences}\gdef\@journalshort{Brain Sci.}\gdef\@doiabbr{brainsci}\gdef\@ISSN{2076-3425}}
\DeclareOption{breath}{\gdef\@journal{breath}\gdef\@journalfull{Breath}\gdef\@journalshort{Breath}\gdef\@doiabbr{breath}\gdef\@ISSN{}}
\DeclareOption{buildings}{\gdef\@journal{buildings}\gdef\@journalfull{Buildings}\gdef\@journalshort{Buildings}\gdef\@doiabbr{buildings}\gdef\@ISSN{2075-5309}}
\DeclareOption{businesses}{\gdef\@journal{businesses}\gdef\@journalfull{Businesses}\gdef\@journalshort{Businesses}\gdef\@doiabbr{businesses}\gdef\@ISSN{2673-7116}\gdef\@continuouspages{yes}}
\DeclareOption{cancers}{\gdef\@journal{cancers}\gdef\@journalfull{Cancers}\gdef\@journalshort{Cancers}\gdef\@doiabbr{cancers}\gdef\@ISSN{2072-6694}}
\DeclareOption{carbon}{\gdef\@journal{carbon}\gdef\@journalfull{C}\gdef\@journalshort{C}\gdef\@doiabbr{c}\gdef\@ISSN{2311-5629}}
\DeclareOption{cardiogenetics}{\gdef\@journal{cardiogenetics}\gdef\@journalfull{Cardiogenetics}\gdef\@journalshort{Cardiogenetics}\gdef\@doiabbr{cardiogenetics}\gdef\@ISSN{2035-8148}\gdef\@continuouspages{yes}}
\DeclareOption{catalysts}{\gdef\@journal{catalysts}\gdef\@journalfull{Catalysts}\gdef\@journalshort{Catalysts}\gdef\@doiabbr{catal}\gdef\@ISSN{2073-4344}}
\DeclareOption{cells}{\gdef\@journal{cells}\gdef\@journalfull{Cells}\gdef\@journalshort{Cells}\gdef\@doiabbr{cells}\gdef\@ISSN{2073-4409}}
\DeclareOption{ceramics}{\gdef\@journal{ceramics}\gdef\@journalfull{Ceramics}\gdef\@journalshort{Ceramics}\gdef\@doiabbr{ceramics}\gdef\@ISSN{2571-6131}\gdef\@continuouspages{yes}}
\DeclareOption{challenges}{\gdef\@journal{challenges}\gdef\@journalfull{Challenges}\gdef\@journalshort{Challenges}\gdef\@doiabbr{challe}\gdef\@ISSN{2078-1547}}
\DeclareOption{chemengineering}{\gdef\@journal{chemengineering}\gdef\@journalfull{ChemEngineering}\gdef\@journalshort{ChemEngineering}\gdef\@doiabbr{chemengineering}\gdef\@ISSN{2305-7084}}
\DeclareOption{chemistry}{\gdef\@journal{chemistry}\gdef\@journalfull{Chemistry}\gdef\@journalshort{Chemistry}\gdef\@doiabbr{chemistry}\gdef\@ISSN{2624-8549}\gdef\@continuouspages{yes}}
\DeclareOption{chemosensors}{\gdef\@journal{chemosensors}\gdef\@journalfull{Chemosensors}\gdef\@journalshort{Chemosensors}\gdef\@doiabbr{chemosensors}\gdef\@ISSN{2227-9040}}
\DeclareOption{chemproc}{\gdef\@journal{chemproc}\gdef\@journalfull{Chemistry Proceedings}\gdef\@journalshort{Chem. Proc.}\gdef\@doiabbr{chemproc}\gdef\@ISSN{2673-4583}}
\DeclareOption{children}{\gdef\@journal{children}\gdef\@journalfull{Children}\gdef\@journalshort{Children}\gdef\@doiabbr{children}\gdef\@ISSN{2227-9067}}
\DeclareOption{chips}{\gdef\@journal{chips}\gdef\@journalfull{Chips}\gdef\@journalshort{Chips}\gdef\@doiabbr{chips}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{cimb}{\gdef\@journal{cimb}\gdef\@journalfull{Current Issues in Molecular Biology}\gdef\@journalshort{Curr. Issues Mol. Biol.}\gdef\@doiabbr{cimb}\gdef\@ISSN{1467-3045}\gdef\@continuouspages{yes}}
\DeclareOption{civileng}{\gdef\@journal{civileng}\gdef\@journalfull{CivilEng}\gdef\@journalshort{CivilEng}\gdef\@doiabbr{civileng}\gdef\@ISSN{2673-4109}\gdef\@continuouspages{yes}}
\DeclareOption{cleantechnol}{\gdef\@journal{cleantechnol}\gdef\@journalfull{Clean Technologies}\gdef\@journalshort{Clean Technol.}\gdef\@doiabbr{cleantechnol}\gdef\@ISSN{2571-8797}\gdef\@continuouspages{yes}}
\DeclareOption{climate}{\gdef\@journal{climate}\gdef\@journalfull{Climate}\gdef\@journalshort{Climate}\gdef\@doiabbr{cli}\gdef\@ISSN{2225-1154}}
\DeclareOption{clinpract}{\gdef\@journal{clinpract}\gdef\@journalfull{Clinics and Practice}\gdef\@journalshort{Clin. Pract.}\gdef\@doiabbr{clinpract}\gdef\@ISSN{2039-7283}\gdef\@continuouspages{yes}}
\DeclareOption{clockssleep}{\gdef\@journal{clockssleep}\gdef\@journalfull{Clocks \& Sleep}\gdef\@journalshort{Clocks\&Sleep}\gdef\@doiabbr{clockssleep}\gdef\@ISSN{2624-5175}\gdef\@continuouspages{yes}}
\DeclareOption{cmd}{\gdef\@journal{cmd}\gdef\@journalfull{Corrosion and Materials Degradation}\gdef\@journalshort{Corros. Mater. Degrad.}\gdef\@doiabbr{cmd}\gdef\@ISSN{2624-5558}\gdef\@continuouspages{yes}}
\DeclareOption{coasts}{\gdef\@journal{coasts}\gdef\@journalfull{Coasts}\gdef\@journalshort{Coasts}\gdef\@doiabbr{coasts}\gdef\@ISSN{2673-964X}\gdef\@continuouspages{yes}}
\DeclareOption{coatings}{\gdef\@journal{coatings}\gdef\@journalfull{Coatings}\gdef\@journalshort{Coatings}\gdef\@doiabbr{coatings}\gdef\@ISSN{2079-6412}}
\DeclareOption{colloids}{\gdef\@journal{colloids}\gdef\@journalfull{Colloids Interfaces}\gdef\@journalshort{Colloids Interfaces}\gdef\@doiabbr{colloids}\gdef\@ISSN{2504-5377}}
\DeclareOption{colorants}{\gdef\@journal{colorants}\gdef\@journalfull{Colorants}\gdef\@journalshort{Colorants}\gdef\@doiabbr{colorants}\gdef\@ISSN{2079-6447}\gdef\@continuouspages{yes}}
\DeclareOption{commodities}{\gdef\@journal{commodities}\gdef\@journalfull{Commodities}\gdef\@journalshort{Commodities}\gdef\@doiabbr{commodities}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{compounds}{\gdef\@journal{compounds}\gdef\@journalfull{Compounds}\gdef\@journalshort{Compounds}\gdef\@doiabbr{compounds}\gdef\@ISSN{2673-6918}\gdef\@continuouspages{yes}}
\DeclareOption{computation}{\gdef\@journal{computation}\gdef\@journalfull{Computation}\gdef\@journalshort{Computation}\gdef\@doiabbr{computation}\gdef\@ISSN{2079-3197}}
\DeclareOption{computers}{\gdef\@journal{computers}\gdef\@journalfull{Computers}\gdef\@journalshort{Computers}\gdef\@doiabbr{computers}\gdef\@ISSN{2073-431X}}
\DeclareOption{condensedmatter}{\gdef\@journal{condensedmatter}\gdef\@journalfull{Condensed Matter}\gdef\@journalshort{Condens. Matter}\gdef\@doiabbr{condmat}\gdef\@ISSN{2410-3896}}
\DeclareOption{conservation}{\gdef\@journal{conservation}\gdef\@journalfull{Conservation}\gdef\@journalshort{Conservation}\gdef\@doiabbr{conservation}\gdef\@ISSN{2673-7159}\gdef\@continuouspages{yes}}
\DeclareOption{constrmater}{\gdef\@journal{constrmater}\gdef\@journalfull{Construction Materials}\gdef\@journalshort{Constr. Mater.}\gdef\@doiabbr{constrmater}\gdef\@ISSN{2673-7108}\gdef\@continuouspages{yes}}
\DeclareOption{cosmetics}{\gdef\@journal{cosmetics}\gdef\@journalfull{Cosmetics}\gdef\@journalshort{Cosmetics}\gdef\@doiabbr{cosmetics}\gdef\@ISSN{2079-9284}}
\DeclareOption{covid}{\gdef\@journal{covid}\gdef\@journalfull{COVID}\gdef\@journalshort{COVID}\gdef\@doiabbr{covid}\gdef\@ISSN{2673-8112}\gdef\@continuouspages{yes}}
\DeclareOption{crops}{\gdef\@journal{crops}\gdef\@journalfull{Crops}\gdef\@journalshort{Crops}\gdef\@doiabbr{crops}\gdef\@ISSN{2673-7655}\gdef\@continuouspages{yes}}
\DeclareOption{cryptography}{\gdef\@journal{cryptography}\gdef\@journalfull{Cryptography}\gdef\@journalshort{Cryptography}\gdef\@doiabbr{cryptography}\gdef\@ISSN{2410-387X}}
\DeclareOption{crystals}{\gdef\@journal{crystals}\gdef\@journalfull{Crystals}\gdef\@journalshort{Crystals}\gdef\@doiabbr{cryst}\gdef\@ISSN{2073-4352}}
\DeclareOption{csmf}{\gdef\@journal{csmf}\gdef\@journalfull{Computer Sciences \& Mathematics Forum}\gdef\@journalshort{Comput. Sci. Math. Forum}\gdef\@doiabbr{csmf}\gdef\@ISSN{2813-0324}}
\DeclareOption{ctn}{\gdef\@journal{ctn}\gdef\@journalfull{Clinical and Translational Neuroscience}\gdef\@journalshort{CTN}\gdef\@doiabbr{Clin. Transl. Neurosci.}\gdef\@ISSN{2514-183X}}
\DeclareOption{curroncol}{\gdef\@journal{curroncol}\gdef\@journalfull{Current Oncology}\gdef\@journalshort{Curr. Oncol.}\gdef\@doiabbr{curroncol}\gdef\@ISSN{1718-7729}\gdef\@continuouspages{yes}}
\DeclareOption{cyber}{\gdef\@journal{cyber}\gdef\@journalfull{Cyber}\gdef\@journalshort{Cyber}\gdef\@doiabbr{cyber}\gdef\@ISSN{2624-800X}}
\DeclareOption{dairy}{\gdef\@journal{dairy}\gdef\@journalfull{Dairy}\gdef\@journalshort{Dairy}\gdef\@doiabbr{dairy}\gdef\@ISSN{2624-862X}\gdef\@continuouspages{yes}}
\DeclareOption{data}{\gdef\@journal{data}\gdef\@journalfull{Data}\gdef\@journalshort{Data}\gdef\@doiabbr{data}\gdef\@ISSN{2306-5729}}
\DeclareOption{dentistry}{\gdef\@journal{dentistry}\gdef\@journalfull{Dentistry Journal}\gdef\@journalshort{Dent. J.}\gdef\@doiabbr{dj}\gdef\@ISSN{2304-6767}}
\DeclareOption{dermato}{\gdef\@journal{dermato}\gdef\@journalfull{Dermato}\gdef\@journalshort{Dermato}\gdef\@doiabbr{dermato}\gdef\@ISSN{2673-6179}\gdef\@continuouspages{yes}}
\DeclareOption{dermatopathology}{\gdef\@journal{dermatopathology}\gdef\@journalfull{Dermatopathology}\gdef\@journalshort{Dermatopathology}\gdef\@doiabbr{dermatopathology}\gdef\@ISSN{2296-3529}\gdef\@continuouspages{yes}}
\DeclareOption{designs}{\gdef\@journal{designs}\gdef\@journalfull{Designs}\gdef\@journalshort{Designs}\gdef\@doiabbr{designs}\gdef\@ISSN{2411-9660}}
\DeclareOption{diabetology}{\gdef\@journal{diabetology}\gdef\@journalfull{Diabetology}\gdef\@journalshort{Diabetology}\gdef\@doiabbr{diabetology}\gdef\@ISSN{2673-4540}\gdef\@continuouspages{yes}}
\DeclareOption{diagnostics}{\gdef\@journal{diagnostics}\gdef\@journalfull{Diagnostics}\gdef\@journalshort{Diagnostics}\gdef\@doiabbr{diagnostics}\gdef\@ISSN{2075-4418}}
\DeclareOption{dietetics}{\gdef\@journal{dietetics}\gdef\@journalfull{Dietetics}\gdef\@journalshort{Dietetics}\gdef\@doiabbr{dietetics}\gdef\@ISSN{2674-0311}\gdef\@continuouspages{yes}}
\DeclareOption{digital}{\gdef\@journal{digital}\gdef\@journalfull{Digital}\gdef\@journalshort{Digital}\gdef\@doiabbr{digital}\gdef\@ISSN{2673-6470}\gdef\@continuouspages{yes}}
\DeclareOption{disabilities}{\gdef\@journal{disabilities}\gdef\@journalfull{Disabilities}\gdef\@journalshort{Disabilities}\gdef\@doiabbr{disabilities}\gdef\@ISSN{2673-7272}\gdef\@continuouspages{yes}}
\DeclareOption{diseases}{\gdef\@journal{diseases}\gdef\@journalfull{Diseases}\gdef\@journalshort{Diseases}\gdef\@doiabbr{diseases}\gdef\@ISSN{2079-9721}}
\DeclareOption{diversity}{\gdef\@journal{diversity}\gdef\@journalfull{Diversity}\gdef\@journalshort{Diversity}\gdef\@doiabbr{d}\gdef\@ISSN{1424-2818}}
\DeclareOption{dna}{\gdef\@journal{dna}\gdef\@journalfull{DNA}\gdef\@journalshort{DNA}\gdef\@doiabbr{dna}\gdef\@ISSN{2673-8856}\gdef\@continuouspages{yes}}
\DeclareOption{drones}{\gdef\@journal{drones}\gdef\@journalfull{Drones}\gdef\@journalshort{Drones}\gdef\@doiabbr{drones}\gdef\@ISSN{2504-446X}}
\DeclareOption{dynamics}{\gdef\@journal{dynamics}\gdef\@journalfull{Dynamics}\gdef\@journalshort{Dynamics}\gdef\@doiabbr{dynamics}\gdef\@ISSN{2673-8716}\gdef\@continuouspages{yes}}
\DeclareOption{earth}{\gdef\@journal{earth}\gdef\@journalfull{Earth}\gdef\@journalshort{Earth}\gdef\@doiabbr{earth}\gdef\@ISSN{2673-4834}\gdef\@continuouspages{yes}}
\DeclareOption{ebj}{\gdef\@journal{ebj}\gdef\@journalfull{European Burn Journal}\gdef\@journalshort{Eur. Burn J.}\gdef\@doiabbr{ebj}\gdef\@ISSN{2673-1991}\gdef\@continuouspages{yes}}
\DeclareOption{ecologies}{\gdef\@journal{ecologies}\gdef\@journalfull{Ecologies}\gdef\@journalshort{Ecologies}\gdef\@doiabbr{ecologies}\gdef\@ISSN{2673-4133}\gdef\@continuouspages{yes}}
\DeclareOption{econometrics}{\gdef\@journal{econometrics}\gdef\@journalfull{Econometrics}\gdef\@journalshort{Econometrics}\gdef\@doiabbr{econometrics}\gdef\@ISSN{2225-1146}}
\DeclareOption{economies}{\gdef\@journal{economies}\gdef\@journalfull{Economies}\gdef\@journalshort{Economies}\gdef\@doiabbr{economies}\gdef\@ISSN{2227-7099}}
\DeclareOption{education}{\gdef\@journal{education}\gdef\@journalfull{Education Sciences}\gdef\@journalshort{Educ. Sci.}\gdef\@doiabbr{educsci}\gdef\@ISSN{2227-7102}}
\DeclareOption{ejihpe}{\gdef\@journal{ejihpe}\gdef\@journalfull{European Journal of Investigation in Health Psychology and Education}\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}\gdef\@doiabbr{ejihpe}\gdef\@ISSN{2254-9625}\gdef\@continuouspages{yes}}
\DeclareOption{electricity}{\gdef\@journal{electricity}\gdef\@journalfull{Electricity}\gdef\@journalshort{Electricity}\gdef\@doiabbr{electricity}\gdef\@ISSN{2673-4826}\gdef\@continuouspages{yes}}
\DeclareOption{electrochem}{\gdef\@journal{electrochem}\gdef\@journalfull{Electrochem}\gdef\@journalshort{Electrochem}\gdef\@doiabbr{electrochem}\gdef\@ISSN{2673-3293}\gdef\@continuouspages{yes}}
\DeclareOption{electronicmat}{\gdef\@journal{electronicmat}\gdef\@journalfull{Electronic Materials}\gdef\@journalshort{Electron. Mater.}\gdef\@doiabbr{electronicmat}\gdef\@ISSN{2673-3978}\gdef\@continuouspages{yes}}
\DeclareOption{electronics}{\gdef\@journal{electronics}\gdef\@journalfull{Electronics}\gdef\@journalshort{Electronics}\gdef\@doiabbr{electronics}\gdef\@ISSN{2079-9292}}
\DeclareOption{encyclopedia}{\gdef\@journal{encyclopedia}\gdef\@journalfull{Encyclopedia}\gdef\@journalshort{Encyclopedia}\gdef\@doiabbr{encyclopedia}\gdef\@ISSN{2673-8392}\gdef\@continuouspages{yes}}
\DeclareOption{endocrines}{\gdef\@journal{endocrines}\gdef\@journalfull{Endocrines}\gdef\@journalshort{Endocrines}\gdef\@doiabbr{endocrines}\gdef\@ISSN{2673-396X}\gdef\@continuouspages{yes}}
\DeclareOption{energies}{\gdef\@journal{energies}\gdef\@journalfull{Energies}\gdef\@journalshort{Energies}\gdef\@doiabbr{en}\gdef\@ISSN{1996-1073}}
\DeclareOption{eng}{\gdef\@journal{eng}\gdef\@journalfull{Eng-Advances in Engineering}\gdef\@journalshort{Eng}\gdef\@doiabbr{eng}\gdef\@ISSN{2673-4117}\gdef\@continuouspages{yes}}
\DeclareOption{engproc}{\gdef\@journal{engproc}\gdef\@journalfull{Engineering Proceedings}\gdef\@journalshort{Eng. Proc.}\gdef\@doiabbr{engproc}\gdef\@ISSN{2673-4591}}
%\DeclareOption{ent}{\gdef\@journal{ent}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{entomology}{\gdef\@journal{entomology}\gdef\@journalfull{Entomology}\gdef\@journalshort{Entomology}\gdef\@doiabbr{entomology}\gdef\@ISSN{2813-0502}\gdef\@continuouspages{yes}}	
\DeclareOption{entropy}{\gdef\@journal{entropy}\gdef\@journalfull{Entropy}\gdef\@journalshort{Entropy}\gdef\@doiabbr{e}\gdef\@ISSN{1099-4300}}
\DeclareOption{environments}{\gdef\@journal{environments}\gdef\@journalfull{Environments}\gdef\@journalshort{Environments}\gdef\@doiabbr{environments}\gdef\@ISSN{2076-3298}}
\DeclareOption{environsciproc}{\gdef\@journal{environsciproc}\gdef\@journalfull{Environmental Sciences Proceedings}\gdef\@journalshort{Environ. Sci. Proc.}\gdef\@doiabbr{environsciproc}\gdef\@ISSN{2673-4931}}
\DeclareOption{epidemiologia}{\gdef\@journal{epidemiologia}\gdef\@journalfull{Epidemiologia}\gdef\@journalshort{Epidemiologia}\gdef\@doiabbr{epidemiologia}\gdef\@ISSN{2673-3986}\gdef\@continuouspages{yes}}
\DeclareOption{epigenomes}{\gdef\@journal{epigenomes}\gdef\@journalfull{Epigenomes}\gdef\@journalshort{Epigenomes}\gdef\@doiabbr{epigenomes}\gdef\@ISSN{2075-4655}}
\DeclareOption{est}{\gdef\@journal{est}\gdef\@journalfull{Electrochemical Science and Technology}\gdef\@journalshort{Electrochem. Sci. Technol.}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{fermentation}{\gdef\@journal{fermentation}\gdef\@journalfull{Fermentation}\gdef\@journalshort{Fermentation}\gdef\@doiabbr{fermentation}\gdef\@ISSN{2311-5637}}
\DeclareOption{fibers}{\gdef\@journal{fibers}\gdef\@journalfull{Fibers}\gdef\@journalshort{Fibers}\gdef\@doiabbr{fib}\gdef\@ISSN{2079-6439}}
\DeclareOption{fintech}{\gdef\@journal{fintech}\gdef\@journalfull{FinTech}\gdef\@journalshort{FinTech}\gdef\@doiabbr{fintech}\gdef\@ISSN{2674-1032}\gdef\@continuouspages{yes}}
\DeclareOption{fire}{\gdef\@journal{fire}\gdef\@journalfull{Fire}\gdef\@journalshort{Fire}\gdef\@doiabbr{fire}\gdef\@ISSN{2571-6255}}
\DeclareOption{fishes}{\gdef\@journal{fishes}\gdef\@journalfull{Fishes}\gdef\@journalshort{Fishes}\gdef\@doiabbr{fishes}\gdef\@ISSN{2410-3888}}
\DeclareOption{fluids}{\gdef\@journal{fluids}\gdef\@journalfull{Fluids}\gdef\@journalshort{Fluids}\gdef\@doiabbr{fluids}\gdef\@ISSN{2311-5521}}
\DeclareOption{foods}{\gdef\@journal{foods}\gdef\@journalfull{Foods}\gdef\@journalshort{Foods}\gdef\@doiabbr{foods}\gdef\@ISSN{2304-8158}}
\DeclareOption{forecasting}{\gdef\@journal{forecasting}\gdef\@journalfull{Forecasting}\gdef\@journalshort{Forecasting}\gdef\@doiabbr{forecast}\gdef\@ISSN{2571-9394}\gdef\@continuouspages{yes}}
\DeclareOption{forensicsci}{\gdef\@journal{forensicsci}\gdef\@journalfull{Forensic Sciences}\gdef\@journalshort{Forensic Sci.}\gdef\@doiabbr{forensicsci}\gdef\@ISSN{2673-6756}\gdef\@continuouspages{yes}}
\DeclareOption{forests}{\gdef\@journal{forests}\gdef\@journalfull{Forests}\gdef\@journalshort{Forests}\gdef\@doiabbr{f}\gdef\@ISSN{1999-4907}}
\DeclareOption{foundations}{\gdef\@journal{foundations}\gdef\@journalfull{Foundations}\gdef\@journalshort{Foundations}\gdef\@doiabbr{foundations}\gdef\@ISSN{2673-9321}\gdef\@continuouspages{yes}}
\DeclareOption{fractalfract}{\gdef\@journal{fractalfract}\gdef\@journalfull{Fractal and Fractional}\gdef\@journalshort{Fractal Fract.}\gdef\@doiabbr{fractalfract}\gdef\@ISSN{2504-3110}}
\DeclareOption{fuels}{\gdef\@journal{fuels}\gdef\@journalfull{Fuels}\gdef\@journalshort{Fuels}\gdef\@doiabbr{fuels}\gdef\@ISSN{2673-3994}\gdef\@continuouspages{yes}}
\DeclareOption{futureinternet}{\gdef\@journal{futureinternet}\gdef\@journalfull{Future Internet}\gdef\@journalshort{Future Internet}\gdef\@doiabbr{fi}\gdef\@ISSN{1999-5903}}
%\DeclareOption{futureparasites}{\gdef\@journal{futureparasites}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{futurepharmacol}{\gdef\@journal{futurepharmacol}\gdef\@journalfull{Future Pharmacology}\gdef\@journalshort{Future Pharm.}\gdef\@doiabbr{futurepharmacol}\gdef\@ISSN{2673-9879}\gdef\@continuouspages{yes}}
\DeclareOption{futurephys}{\gdef\@journal{futurephys}\gdef\@journalfull{Future Physics}\gdef\@journalshort{Future Phys.}\gdef\@doiabbr{futurephys}\gdef\@ISSN{2624-6503}}
\DeclareOption{futuretransp}{\gdef\@journal{futuretransp}\gdef\@journalfull{Future Transportation}\gdef\@journalshort{Future Transp.}\gdef\@doiabbr{futuretransp}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{galaxies}{\gdef\@journal{galaxies}\gdef\@journalfull{Galaxies}\gdef\@journalshort{Galaxies}\gdef\@doiabbr{galaxies}\gdef\@ISSN{2075-4434}}
\DeclareOption{games}{\gdef\@journal{games}\gdef\@journalfull{Games}\gdef\@journalshort{Games}\gdef\@doiabbr{g}\gdef\@ISSN{2073-4336}}
\DeclareOption{gases}{\gdef\@journal{gases}\gdef\@journalfull{Gases}\gdef\@journalshort{Gases}\gdef\@doiabbr{gases}\gdef\@ISSN{2673-5628}\gdef\@continuouspages{yes}}
\DeclareOption{gastroent}{\gdef\@journal{gastroent}\gdef\@journalfull{Gastroenterology Insights}\gdef\@journalshort{Gastroenterol. Insights}\gdef\@doiabbr{gastroent}\gdef\@ISSN{2036-7422}\gdef\@continuouspages{yes}}
\DeclareOption{gastrointestdisord}{\gdef\@journal{gastrointestdisord}\gdef\@journalfull{Gastrointestinal Disorders}\gdef\@journalshort{Gastrointest. Disord.}\gdef\@doiabbr{gidisord}\gdef\@ISSN{2624-5647}\gdef\@continuouspages{yes}}
\DeclareOption{gels}{\gdef\@journal{gels}\gdef\@journalfull{Gels}\gdef\@journalshort{Gels}\gdef\@doiabbr{gels}\gdef\@ISSN{2310-2861}}
\DeclareOption{genealogy}{\gdef\@journal{genealogy}\gdef\@journalfull{Genealogy}\gdef\@journalshort{Genealogy}\gdef\@doiabbr{genealogy}\gdef\@ISSN{2313-5778}}
\DeclareOption{genes}{\gdef\@journal{genes}\gdef\@journalfull{Genes}\gdef\@journalshort{Genes}\gdef\@doiabbr{genes}\gdef\@ISSN{2073-4425}}
\DeclareOption{geographies}{\gdef\@journal{geographies}\gdef\@journalfull{Geographies}\gdef\@journalshort{Geographies}\gdef\@doiabbr{geographies}\gdef\@ISSN{2673-7086}\gdef\@continuouspages{yes}}
\DeclareOption{geohazards}{\gdef\@journal{geohazards}\gdef\@journalfull{GeoHazards}\gdef\@journalshort{GeoHazards}\gdef\@doiabbr{geohazards}\gdef\@ISSN{2624-795X}\gdef\@continuouspages{yes}}
\DeclareOption{geomatics}{\gdef\@journal{geomatics}\gdef\@journalfull{Geomatics}\gdef\@journalshort{Geomatics}\gdef\@doiabbr{geomatics}\gdef\@ISSN{2673-7418}\gdef\@continuouspages{yes}}
\DeclareOption{geosciences}{\gdef\@journal{geosciences}\gdef\@journalfull{Geosciences}\gdef\@journalshort{Geosciences}\gdef\@doiabbr{geosciences}\gdef\@ISSN{2076-3263}}
\DeclareOption{geotechnics}{\gdef\@journal{geotechnics}\gdef\@journalfull{Geotechnics}\gdef\@journalshort{Geotechnics}\gdef\@doiabbr{geotechnics}\gdef\@ISSN{2673-7094}\gdef\@continuouspages{yes}}
\DeclareOption{geriatrics}{\gdef\@journal{geriatrics}\gdef\@journalfull{Geriatrics}\gdef\@journalshort{Geriatrics}\gdef\@doiabbr{geriatrics}\gdef\@ISSN{2308-3417}}
\DeclareOption{grasses}{\gdef\@journal{grasses}\gdef\@journalfull{Grasses}\gdef\@journalshort{Grasses}\gdef\@doiabbr{grasses}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hazardousmatters}{\gdef\@journal{hazardousmatters}\gdef\@journalfull{Hazardous Matters}\gdef\@journalshort{Hazard. Matters}\gdef\@doiabbr{}\gdef\@ISSN{0014-0014}}
\DeclareOption{healthcare}{\gdef\@journal{healthcare}\gdef\@journalfull{Healthcare}\gdef\@journalshort{Healthcare}\gdef\@doiabbr{healthcare}\gdef\@ISSN{2227-9032}}
\DeclareOption{hearts}{\gdef\@journal{hearts}\gdef\@journalfull{Hearts}\gdef\@journalshort{Hearts}\gdef\@doiabbr{hearts}\gdef\@ISSN{2673-3846}\gdef\@continuouspages{yes}}
\DeclareOption{hemato}{\gdef\@journal{hemato}\gdef\@journalfull{Hemato}\gdef\@journalshort{Hemato}\gdef\@doiabbr{hemato}\gdef\@ISSN{2673-6357}\gdef\@continuouspages{yes}}
\DeclareOption{hematolrep}{\gdef\@journal{hematolrep}\gdef\@journalfull{Hematology Reports}\gdef\@journalshort{Hematol. Rep.}\gdef\@doiabbr{hematolrep}\gdef\@ISSN{2038-8330}\gdef\@continuouspages{yes}}
\DeclareOption{heritage}{\gdef\@journal{heritage}\gdef\@journalfull{Heritage}\gdef\@journalshort{Heritage}\gdef\@doiabbr{heritage}\gdef\@ISSN{2571-9408}\gdef\@continuouspages{yes}}
\DeclareOption{highthroughput}{\gdef\@journal{highthroughput}\gdef\@journalfull{High-Throughput}\gdef\@journalshort{High-Throughput}\gdef\@doiabbr{ht}\gdef\@ISSN{2571-5135}}
\DeclareOption{histories}{\gdef\@journal{histories}\gdef\@journalfull{Histories}\gdef\@journalshort{Histories}\gdef\@doiabbr{histories}\gdef\@ISSN{2409-9252}\gdef\@continuouspages{yes}}
\DeclareOption{horticulturae}{\gdef\@journal{horticulturae}\gdef\@journalfull{Horticulturae}\gdef\@journalshort{Horticulturae}\gdef\@doiabbr{horticulturae}\gdef\@ISSN{2311-7524}}
\DeclareOption{humanities}{\gdef\@journal{humanities}\gdef\@journalfull{Humanities}\gdef\@journalshort{Humanities}\gdef\@doiabbr{h}\gdef\@ISSN{2076-0787}}
\DeclareOption{humans}{\gdef\@journal{humans}\gdef\@journalfull{Humans}\gdef\@journalshort{Humans}\gdef\@doiabbr{humans}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hydrobiology}{\gdef\@journal{hydrobiology}\gdef\@journalfull{Hydrobiology}\gdef\@journalshort{Hydrobiology	}\gdef\@doiabbr{hydrobiology}\gdef\@ISSN{2673-9917}\gdef\@continuouspages{yes}}
\DeclareOption{hydrogen}{\gdef\@journal{hydrogen}\gdef\@journalfull{Hydrogen}\gdef\@journalshort{Hydrogen}\gdef\@doiabbr{hydrogen}\gdef\@ISSN{2673-4141}\gdef\@continuouspages{yes}}
\DeclareOption{hydrology}{\gdef\@journal{hydrology}\gdef\@journalfull{Hydrology}\gdef\@journalshort{Hydrology}\gdef\@doiabbr{hydrology}\gdef\@ISSN{2306-5338}}
\DeclareOption{hygiene}{\gdef\@journal{hygiene}\gdef\@journalfull{Hygiene}\gdef\@journalshort{Hygiene}\gdef\@doiabbr{hygiene}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{idr}{\gdef\@journal{idr}\gdef\@journalfull{Infectious Disease Reports}\gdef\@journalshort{Infect. Dis. Rep.}\gdef\@doiabbr{idr}\gdef\@ISSN{2036-7449}\gdef\@continuouspages{yes}}
\DeclareOption{ijerph}{\gdef\@journal{ijerph}\gdef\@journalfull{International Journal of Environmental Research and Public Health}\gdef\@journalshort{Int. J. Environ. Res. Public Health}\gdef\@doiabbr{ijerph}\gdef\@ISSN{1660-4601}}
\DeclareOption{ijfs}{\gdef\@journal{ijfs}\gdef\@journalfull{International Journal of Financial Studies}\gdef\@journalshort{Int. J. Financial Stud.}\gdef\@doiabbr{ijfs}\gdef\@ISSN{2227-7072}}
\DeclareOption{ijgi}{\gdef\@journal{ijgi}\gdef\@journalfull{ISPRS International Journal of Geo-Information}\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}\gdef\@doiabbr{ijgi}\gdef\@ISSN{2220-9964}}
\DeclareOption{ijms}{\gdef\@journal{ijms}\gdef\@journalfull{International Journal of Molecular Sciences}\gdef\@journalshort{Int. J. Mol. Sci.}\gdef\@doiabbr{ijms}\gdef\@ISSN{1422-0067}}
\DeclareOption{ijns}{\gdef\@journal{ijns}\gdef\@journalfull{International Journal of Neonatal Screening}\gdef\@journalshort{Int. J. Neonatal Screen.}\gdef\@doiabbr{ijns}\gdef\@ISSN{2409-515X}}
\DeclareOption{ijpb}{\gdef\@journal{ijpb}\gdef\@journalfull{International Journal of Plant Biology}\gdef\@journalshort{Int. J. Plant Biol.}\gdef\@doiabbr{ijpb}\gdef\@ISSN{2037-0164}\gdef\@continuouspages{yes}}
\DeclareOption{ijtm}{\gdef\@journal{ijtm}\gdef\@journalfull{International Journal of Translational Medicine}\gdef\@journalshort{Int. J. Transl. Med.}\gdef\@doiabbr{ijtm}\gdef\@ISSN{2673-8937}\gdef\@continuouspages{yes}}
\DeclareOption{ijtpp}{\gdef\@journal{ijtpp}\gdef\@journalfull{International Journal of Turbomachinery Propulsion and Power}\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}\gdef\@doiabbr{ijtpp}\gdef\@ISSN{2504-186X}}
\DeclareOption{ime}{\gdef\@journal{ime}\gdef\@journalfull{International Medical Education}\gdef\@journalshort{Int. Med. Educ.}\gdef\@doiabbr{ime}\gdef\@ISSN{2813-141X}\gdef\@continuouspages{yes}}
\DeclareOption{immuno}{\gdef\@journal{immuno}\gdef\@journalfull{Immuno}\gdef\@journalshort{Immuno}\gdef\@doiabbr{immuno}\gdef\@ISSN{2673-5601}\gdef\@continuouspages{yes}}
\DeclareOption{informatics}{\gdef\@journal{informatics}\gdef\@journalfull{Informatics}\gdef\@journalshort{Informatics}\gdef\@doiabbr{informatics}\gdef\@ISSN{2227-9709}}
\DeclareOption{information}{\gdef\@journal{information}\gdef\@journalfull{Information}\gdef\@journalshort{Information}\gdef\@doiabbr{info}\gdef\@ISSN{2078-2489}}
\DeclareOption{infrastructures}{\gdef\@journal{infrastructures}\gdef\@journalfull{Infrastructures}\gdef\@journalshort{Infrastructures}\gdef\@doiabbr{infrastructures}\gdef\@ISSN{2412-3811}}
\DeclareOption{inorganics}{\gdef\@journal{inorganics}\gdef\@journalfull{Inorganics}\gdef\@journalshort{Inorganics}\gdef\@doiabbr{inorganics}\gdef\@ISSN{2304-6740}}
\DeclareOption{insects}{\gdef\@journal{insects}\gdef\@journalfull{Insects}\gdef\@journalshort{Insects}\gdef\@doiabbr{insects}\gdef\@ISSN{2075-4450}}
\DeclareOption{instruments}{\gdef\@journal{instruments}\gdef\@journalfull{Instruments}\gdef\@journalshort{Instruments}\gdef\@doiabbr{instruments}\gdef\@ISSN{2410-390X}}
\DeclareOption{inventions}{\gdef\@journal{inventions}\gdef\@journalfull{Inventions}\gdef\@journalshort{Inventions}\gdef\@doiabbr{inventions}\gdef\@ISSN{2411-5134}}
\DeclareOption{iot}{\gdef\@journal{iot}\gdef\@journalfull{IoT}\gdef\@journalshort{IoT}\gdef\@doiabbr{iot}\gdef\@ISSN{2624-831X}\gdef\@continuouspages{yes}}
\DeclareOption{j}{\gdef\@journal{j}\gdef\@journalfull{J}\gdef\@journalshort{J}\gdef\@doiabbr{j}\gdef\@ISSN{2571-8800}\gdef\@continuouspages{yes}}
\DeclareOption{jal}{\gdef\@journal{jal}\gdef\@journalfull{Journal of Ageing and Longevity}\gdef\@journalshort{J. Ageing Longev.}\gdef\@doiabbr{jal}\gdef\@ISSN{2673-9259}\gdef\@continuouspages{yes}}
\DeclareOption{jcdd}{\gdef\@journal{jcdd}\gdef\@journalfull{Journal of Cardiovascular Development and Disease}\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}\gdef\@doiabbr{jcdd}\gdef\@ISSN{2308-3425}}
\DeclareOption{jcm}{\gdef\@journal{jcm}\gdef\@journalfull{Journal of Clinical Medicine}\gdef\@journalshort{J. Clin. Med.}\gdef\@doiabbr{jcm}\gdef\@ISSN{2077-0383}}
\DeclareOption{jcp}{\gdef\@journal{jcp}\gdef\@journalfull{Journal of Cybersecurity and Privacy}\gdef\@journalshort{J. Cybersecur. Priv.}\gdef\@doiabbr{jcp}\gdef\@ISSN{2624-800X}\gdef\@continuouspages{yes}}
\DeclareOption{jcs}{\gdef\@journal{jcs}\gdef\@journalfull{Journal of Composites Science}\gdef\@journalshort{J. Compos. Sci.}\gdef\@doiabbr{jcs}\gdef\@ISSN{2504-477X}}
\DeclareOption{jcto}{\gdef\@journal{jcto}\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}\gdef\@doiabbr{jcto}\gdef\@ISSN{2813-1053}\gdef\@continuouspages{yes}}
\DeclareOption{jdb}{\gdef\@journal{jdb}\gdef\@journalfull{Journal of Developmental Biology}\gdef\@journalshort{J. Dev. Biol.}\gdef\@doiabbr{jdb}\gdef\@ISSN{2221-3759}}
\DeclareOption{jeta}{\gdef\@journal{jeta}\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}\gdef\@journalshort{J. Exp. Theor. Anal.}\gdef\@doiabbr{jeta}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jfb}{\gdef\@journal{jfb}\gdef\@journalfull{Journal of Functional Biomaterials}\gdef\@journalshort{J. Funct. Biomater.}\gdef\@doiabbr{jfb}\gdef\@ISSN{2079-4983}}
\DeclareOption{jfmk}{\gdef\@journal{jfmk}\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}\gdef\@doiabbr{jfmk}\gdef\@ISSN{2411-5142}}
\DeclareOption{jimaging}{\gdef\@journal{jimaging}\gdef\@journalfull{Journal of Imaging}\gdef\@journalshort{J. Imaging}\gdef\@doiabbr{jimaging}\gdef\@ISSN{2313-433X}}
\DeclareOption{jintelligence}{\gdef\@journal{jintelligence}\gdef\@journalfull{Journal of Intelligence}\gdef\@journalshort{J. Intell.}\gdef\@doiabbr{jintelligence}\gdef\@ISSN{2079-3200}}
\DeclareOption{jlpea}{\gdef\@journal{jlpea}\gdef\@journalfull{Journal of Low Power Electronics and Applications}\gdef\@journalshort{J. Low Power Electron. Appl.}\gdef\@doiabbr{jlpea}\gdef\@ISSN{2079-9268}}
\DeclareOption{jmmp}{\gdef\@journal{jmmp}\gdef\@journalfull{Journal of Manufacturing and Materials Processing}\gdef\@journalshort{J. Manuf. Mater. Process.}\gdef\@doiabbr{jmmp}\gdef\@ISSN{2504-4494}}
\DeclareOption{jmp}{\gdef\@journal{jmp}\gdef\@journalfull{Journal of Molecular Pathology}\gdef\@journalshort{J. Mol. Pathol.}\gdef\@doiabbr{jmp}\gdef\@ISSN{2673-5261}\gdef\@continuouspages{yes}}
\DeclareOption{jmse}{\gdef\@journal{jmse}\gdef\@journalfull{Journal of Marine Science and Engineering}\gdef\@journalshort{J. Mar. Sci. Eng.}\gdef\@doiabbr{jmse}\gdef\@ISSN{2077-1312}}
\DeclareOption{jne}{\gdef\@journal{jne}\gdef\@journalfull{Journal of Nuclear Engineering}\gdef\@journalshort{J. Nucl. Eng.}\gdef\@doiabbr{jne}\gdef\@ISSN{2673-4362}\gdef\@continuouspages{yes}}
\DeclareOption{jnt}{\gdef\@journal{jnt}\gdef\@journalfull{Journal of Nanotheranostics}\gdef\@journalshort{J. Nanotheranostics}\gdef\@doiabbr{jnt}\gdef\@ISSN{2624-845X}\gdef\@continuouspages{yes}}
\DeclareOption{jof}{\gdef\@journal{jof}\gdef\@journalfull{Journal of Fungi}\gdef\@journalshort{J. Fungi}\gdef\@doiabbr{jof}\gdef\@ISSN{2309-608X}}
\DeclareOption{joitmc}{\gdef\@journal{joitmc}\gdef\@journalfull{Journal of Open Innovation: Technology Market and Complexity}\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}\gdef\@doiabbr{joitmc}\gdef\@ISSN{2199-8531}}
\DeclareOption{jor}{\gdef\@journal{jor}\gdef\@journalfull{Journal of Respiration}\gdef\@journalshort{J. Respir.}\gdef\@doiabbr{jor}\gdef\@ISSN{2673-527X}\gdef\@continuouspages{yes}}
\DeclareOption{journalmedia}{\gdef\@journal{journalmedia}\gdef\@journalfull{Journalism and Media}\gdef\@journalshort{Journal. Media}\gdef\@doiabbr{journalmedia}\gdef\@ISSN{2673-5172}\gdef\@continuouspages{yes}}
\DeclareOption{jox}{\gdef\@journal{jox}\gdef\@journalfull{Journal of Xenobiotics}\gdef\@journalshort{J. Xenobiot.}\gdef\@doiabbr{jox}\gdef\@ISSN{2039-4713}\gdef\@continuouspages{yes}}
\DeclareOption{jpm}{\gdef\@journal{jpm}\gdef\@journalfull{Journal of Personalized Medicine}\gdef\@journalshort{J. Pers. Med.}\gdef\@doiabbr{jpm}\gdef\@ISSN{2075-4426}}
\DeclareOption{jrfm}{\gdef\@journal{jrfm}\gdef\@journalfull{Journal of Risk and Financial Management}\gdef\@journalshort{J. Risk Financial Manag.}\gdef\@doiabbr{jrfm}\gdef\@ISSN{1911-8074}}
\DeclareOption{jsan}{\gdef\@journal{jsan}\gdef\@journalfull{Journal of Sensor and Actuator Networks}\gdef\@journalshort{J. Sens. Actuator Netw.}\gdef\@doiabbr{jsan}\gdef\@ISSN{2224-2708}}
\DeclareOption{jtaer}{\gdef\@journal{jtaer}\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}\gdef\@doiabbr{jtaer}\gdef\@ISSN{0718-1876}\gdef\@continuouspages{yes}}
\DeclareOption{jvd}{\gdef\@journal{jvd}\gdef\@journalfull{Journal of Vascular Diseases}\gdef\@journalshort{JVD}\gdef\@doiabbr{jvd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jzbg}{\gdef\@journal{jzbg}\gdef\@journalfull{Journal of Zoological and Botanical Gardens}\gdef\@journalshort{J. Zool. Bot. Gard.}\gdef\@doiabbr{jzbg}\gdef\@ISSN{2673-5636}\gdef\@continuouspages{yes}}
%\DeclareOption{kidney}{\gdef\@journal{kidney}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kidneydial}{\gdef\@journal{kidneydial}\gdef\@journalfull{Kidney and Dialysis}\gdef\@journalshort{Kidney Dial.}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kinasesphosphatases}{\gdef\@journal{kinasesphosphatases}\gdef\@journalfull{Kinases and Phosphatases}\gdef\@journalshort{Kinases Phosphatases}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{knowledge}{\gdef\@journal{knowledge}\gdef\@journalfull{Knowledge}\gdef\@journalshort{Knowledge}\gdef\@doiabbr{knowledge}\gdef\@ISSN{2673-9585}\gdef\@continuouspages{yes}}
\DeclareOption{land}{\gdef\@journal{land}\gdef\@journalfull{Land}\gdef\@journalshort{Land}\gdef\@doiabbr{land}\gdef\@ISSN{2073-445X}}
\DeclareOption{languages}{\gdef\@journal{languages}\gdef\@journalfull{Languages}\gdef\@journalshort{Languages}\gdef\@doiabbr{languages}\gdef\@ISSN{2226-471X}}
\DeclareOption{laws}{\gdef\@journal{laws}\gdef\@journalfull{Laws}\gdef\@journalshort{Laws}\gdef\@doiabbr{laws}\gdef\@ISSN{2075-471X}}
\DeclareOption{life}{\gdef\@journal{life}\gdef\@journalfull{Life}\gdef\@journalshort{Life}\gdef\@doiabbr{life}\gdef\@ISSN{2075-1729}}
\DeclareOption{liquids}{\gdef\@journal{liquids}\gdef\@journalfull{Liquids}\gdef\@journalshort{Liquids}\gdef\@doiabbr{liquids}\gdef\@ISSN{2673-8015}\gdef\@continuouspages{yes}}
\DeclareOption{literature}{\gdef\@journal{literature}\gdef\@journalfull{Literature}\gdef\@journalshort{Literature}\gdef\@doiabbr{literature}\gdef\@ISSN{2410-9789}\gdef\@continuouspages{yes}}
\DeclareOption{livers}{\gdef\@journal{livers}\gdef\@journalfull{Livers}\gdef\@journalshort{Livers}\gdef\@doiabbr{livers}\gdef\@ISSN{2673-4389}\gdef\@continuouspages{yes}}
\DeclareOption{logics}{\gdef\@journal{logics}\gdef\@journalfull{Logics}\gdef\@journalshort{Logics}\gdef\@doiabbr{logics}\gdef\@ISSN{2813-0405}\gdef\@continuouspages{yes}}
\DeclareOption{logistics}{\gdef\@journal{logistics}\gdef\@journalfull{Logistics}\gdef\@journalshort{Logistics}\gdef\@doiabbr{logistics}\gdef\@ISSN{2305-6290}}
\DeclareOption{lubricants}{\gdef\@journal{lubricants}\gdef\@journalfull{Lubricants}\gdef\@journalshort{Lubricants}\gdef\@doiabbr{lubricants}\gdef\@ISSN{2075-4442}}
\DeclareOption{lymphatics}{\gdef\@journal{lymphatics}\gdef\@journalfull{Lymphatics}\gdef\@journalshort{Lymphatics}\gdef\@doiabbr{lymphatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}	
\DeclareOption{machines}{\gdef\@journal{machines}\gdef\@journalfull{Machines}\gdef\@journalshort{Machines}\gdef\@doiabbr{machines}\gdef\@ISSN{2075-1702}}
\DeclareOption{macromol}{\gdef\@journal{macromol}\gdef\@journalfull{Macromol}\gdef\@journalshort{Macromol}\gdef\@doiabbr{macromol}\gdef\@ISSN{2673-6209}\gdef\@continuouspages{yes}}
\DeclareOption{magnetism}{\gdef\@journal{magnetism}\gdef\@journalfull{Magnetism}\gdef\@journalshort{Magnetism}\gdef\@doiabbr{magnetism}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{magnetochemistry}{\gdef\@journal{magnetochemistry}\gdef\@journalfull{Magnetochemistry}\gdef\@journalshort{Magnetochemistry}\gdef\@doiabbr{magnetochemistry}\gdef\@ISSN{2312-7481}}
\DeclareOption{make}{\gdef\@journal{make}\gdef\@journalfull{Machine Learning and Knowledge Extraction}\gdef\@journalshort{Mach. Learn. Knowl. Extr.}\gdef\@doiabbr{make}\gdef\@ISSN{2504-4990}\gdef\@continuouspages{yes}}
\DeclareOption{marinedrugs}{\gdef\@journal{marinedrugs}\gdef\@journalfull{Marine Drugs}\gdef\@journalshort{Mar. Drugs}\gdef\@doiabbr{md}\gdef\@ISSN{1660-3397}}
\DeclareOption{materials}{\gdef\@journal{materials}\gdef\@journalfull{Materials}\gdef\@journalshort{Materials}\gdef\@doiabbr{ma}\gdef\@ISSN{1996-1944}}
\DeclareOption{materproc}{\gdef\@journal{materproc}\gdef\@journalfull{Materials Proceedings}\gdef\@journalshort{Mater. Proc.}\gdef\@doiabbr{materproc}\gdef\@ISSN{2673-4605}}
\DeclareOption{mathematics}{\gdef\@journal{mathematics}\gdef\@journalfull{Mathematics}\gdef\@journalshort{Mathematics}\gdef\@doiabbr{math}\gdef\@ISSN{2227-7390}}
\DeclareOption{mca}{\gdef\@journal{mca}\gdef\@journalfull{Mathematical and Computational Applications}\gdef\@journalshort{Math. Comput. Appl.}\gdef\@doiabbr{mca}\gdef\@ISSN{2297-8747}}
\DeclareOption{measurements}{\gdef\@journal{measurements}\gdef\@journalfull{Measurements}\gdef\@journalshort{Measurements}\gdef\@doiabbr{measurements}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{medicina}{\gdef\@journal{medicina}\gdef\@journalfull{Medicina}\gdef\@journalshort{Medicina}\gdef\@doiabbr{medicina}\gdef\@ISSN{1648-9144}}
\DeclareOption{medicines}{\gdef\@journal{medicines}\gdef\@journalfull{Medicines}\gdef\@journalshort{Medicines}\gdef\@doiabbr{medicines}\gdef\@ISSN{2305-6320}}
\DeclareOption{medsci}{\gdef\@journal{medsci}\gdef\@journalfull{Medical Sciences}\gdef\@journalshort{Med. Sci.}\gdef\@doiabbr{medsci}\gdef\@ISSN{2076-3271}}
\DeclareOption{membranes}{\gdef\@journal{membranes}\gdef\@journalfull{Membranes}\gdef\@journalshort{Membranes}\gdef\@doiabbr{membranes}\gdef\@ISSN{2077-0375}}
\DeclareOption{merits}{\gdef\@journal{merits}\gdef\@journalfull{Merits}\gdef\@journalshort{Merits}\gdef\@doiabbr{merits}\gdef\@ISSN{2673-8104}\gdef\@continuouspages{yes}}
\DeclareOption{metabolites}{\gdef\@journal{metabolites}\gdef\@journalfull{Metabolites}\gdef\@journalshort{Metabolites}\gdef\@doiabbr{metabo}\gdef\@ISSN{2218-1989}}
\DeclareOption{metals}{\gdef\@journal{metals}\gdef\@journalfull{Metals}\gdef\@journalshort{Metals}\gdef\@doiabbr{met}\gdef\@ISSN{2075-4701}}
\DeclareOption{meteorology}{\gdef\@journal{meteorology}\gdef\@journalfull{Meteorology}\gdef\@journalshort{Meteorology}\gdef\@doiabbr{meteorology}\gdef\@ISSN{2674-0494}\gdef\@continuouspages{yes}}
\DeclareOption{methane}{\gdef\@journal{methane}\gdef\@journalfull{Methane}\gdef\@journalshort{Methane}\gdef\@doiabbr{methane}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{metrology}{\gdef\@journal{metrology}\gdef\@journalfull{Metrology}\gdef\@journalshort{Metrology}\gdef\@doiabbr{metrology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{micro}{\gdef\@journal{micro}\gdef\@journalfull{Micro}\gdef\@journalshort{Micro}\gdef\@doiabbr{micro}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{microarrays}{\gdef\@journal{microarrays}\gdef\@journalfull{Microarrays}\gdef\@journalshort{Microarrays}\gdef\@doiabbr{microarrays}\gdef\@ISSN{2076-3905}}
\DeclareOption{microbiolres}{\gdef\@journal{microbiolres}\gdef\@journalfull{Microbiology Research}\gdef\@journalshort{Microbiol. Res.}\gdef\@doiabbr{microbiolres}\gdef\@ISSN{2036-7481}\gdef\@continuouspages{yes}}
\DeclareOption{micromachines}{\gdef\@journal{micromachines}\gdef\@journalfull{Micromachines}\gdef\@journalshort{Micromachines}\gdef\@doiabbr{mi}\gdef\@ISSN{2072-666X}}
\DeclareOption{microorganisms}{\gdef\@journal{microorganisms}\gdef\@journalfull{Microorganisms}\gdef\@journalshort{Microorganisms}\gdef\@doiabbr{microorganisms}\gdef\@ISSN{2076-2607}}
\DeclareOption{microplastics}{\gdef\@journal{microplastics}\gdef\@journalfull{Microplastics}\gdef\@journalshort{Microplastics}\gdef\@doiabbr{microplastics}\gdef\@ISSN{2673-8929}\gdef\@continuouspages{yes}}
\DeclareOption{minerals}{\gdef\@journal{minerals}\gdef\@journalfull{Minerals}\gdef\@journalshort{Minerals}\gdef\@doiabbr{min}\gdef\@ISSN{2075-163X}}
\DeclareOption{mining}{\gdef\@journal{mining}\gdef\@journalfull{Mining}\gdef\@journalshort{Mining}\gdef\@doiabbr{mining}\gdef\@ISSN{2673-6489}\gdef\@continuouspages{yes}}
\DeclareOption{modelling}{\gdef\@journal{modelling}\gdef\@journalfull{Modelling}\gdef\@journalshort{Modelling}\gdef\@doiabbr{modelling}\gdef\@ISSN{2673-3951}\gdef\@continuouspages{yes}}
\DeclareOption{molbank}{\gdef\@journal{molbank}\gdef\@journalfull{Molbank}\gdef\@journalshort{Molbank}\gdef\@doiabbr{M}\gdef\@ISSN{1422-8599}}
\DeclareOption{molecules}{\gdef\@journal{molecules}\gdef\@journalfull{Molecules}\gdef\@journalshort{Molecules}\gdef\@doiabbr{molecules}\gdef\@ISSN{1420-3049}}
\DeclareOption{mps}{\gdef\@journal{mps}\gdef\@journalfull{Methods and Protocols}\gdef\@journalshort{Methods Protoc.}\gdef\@doiabbr{mps}\gdef\@ISSN{2409-9279}}
\DeclareOption{msf}{\gdef\@journal{msf}\gdef\@journalfull{Medical Sciences Forum}\gdef\@journalshort{Med. Sci. Forum}\gdef\@doiabbr{msf}\gdef\@ISSN{2673-9992}}
\DeclareOption{mti}{\gdef\@journal{mti}\gdef\@journalfull{Multimodal Technologies and Interaction}\gdef\@journalshort{Multimodal Technol. Interact.}\gdef\@doiabbr{mti}\gdef\@ISSN{2414-4088}}
\DeclareOption{muscles}{\gdef\@journal{muscles}\gdef\@journalfull{Muscles}\gdef\@journalshort{Muscles}\gdef\@doiabbr{muscles}\gdef\@ISSN{2813-0413}\gdef\@continuouspages{yes}}
\DeclareOption{nanoenergyadv}{\gdef\@journal{nanoenergyadv}\gdef\@journalfull{Nanoenergy Advances}\gdef\@journalshort{Nanoenergy Adv.}\gdef\@doiabbr{nanoenergyadv}\gdef\@ISSN{2673-706X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomanufacturing}{\gdef\@journal{nanomanufacturing}\gdef\@journalfull{Nanomanufacturing}\gdef\@journalshort{Nanomanufacturing}\gdef\@doiabbr{nanomanufacturing}\gdef\@ISSN{2673-687X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomaterials}{\gdef\@journal{nanomaterials}\gdef\@journalfull{Nanomaterials}\gdef\@journalshort{Nanomaterials}\gdef\@doiabbr{nano}\gdef\@ISSN{2079-4991}}
\DeclareOption{ncrna}{\gdef\@journal{ncrna}\gdef\@journalfull{Non-Coding RNA}\gdef\@journalshort{Non-Coding RNA}\gdef\@doiabbr{ncrna}\gdef\@ISSN{2311-553X}}
\DeclareOption{network}{\gdef\@journal{network}\gdef\@journalfull{Network}\gdef\@journalshort{Network}\gdef\@doiabbr{network}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{neuroglia}{\gdef\@journal{neuroglia}\gdef\@journalfull{Neuroglia}\gdef\@journalshort{Neuroglia}\gdef\@doiabbr{neuroglia}\gdef\@ISSN{2571-6980}\gdef\@continuouspages{yes}}
\DeclareOption{neurolint}{\gdef\@journal{neurolint}\gdef\@journalfull{Neurology International}\gdef\@journalshort{Neurol. Int.}\gdef\@doiabbr{neurolint}\gdef\@ISSN{2035-8377}\gdef\@continuouspages{yes}}
\DeclareOption{neurosci}{\gdef\@journal{neurosci}\gdef\@journalfull{NeuroSci}\gdef\@journalshort{NeuroSci}\gdef\@doiabbr{neurosci}\gdef\@ISSN{2673-4087}\gdef\@continuouspages{yes}}
\DeclareOption{nitrogen}{\gdef\@journal{nitrogen}\gdef\@journalfull{Nitrogen}\gdef\@journalshort{Nitrogen}\gdef\@doiabbr{nitrogen}\gdef\@ISSN{2504-3129}\gdef\@continuouspages{yes}}
\DeclareOption{notspecified}{\gdef\@journal{notspecified}\gdef\@journalfull{Journal Not Specified}\gdef\@journalshort{Journal Not Specified}\gdef\@doiabbr{}\gdef\@ISSN{}}
%%\DeclareOption{nri}{\gdef\@journal{nri}\gdef\@journalfull{Natural Resources Informatics}\gdef\@journalshort{Nat. Resour. Inform.}\gdef\@doiabbr{nri}\gdef\@ISSN{2673-981X}\gdef\@continuouspages{yes}}
\DeclareOption{nursrep}{\gdef\@journal{nursrep}\gdef\@journalfull{Nursing Reports}\gdef\@journalshort{Nurs. Rep.}\gdef\@doiabbr{nursrep}\gdef\@ISSN{2039-4403}\gdef\@continuouspages{yes}}
\DeclareOption{nutraceuticals}{\gdef\@journal{nutraceuticals}\gdef\@journalfull{Nutraceuticals}\gdef\@journalshort{Nutraceuticals}\gdef\@doiabbr{nutraceuticals}\gdef\@ISSN{1661-3821}\gdef\@continuouspages{yes}}
\DeclareOption{nutrients}{\gdef\@journal{nutrients}\gdef\@journalfull{Nutrients}\gdef\@journalshort{Nutrients}\gdef\@doiabbr{nu}\gdef\@ISSN{2072-6643}}
\DeclareOption{obesities}{\gdef\@journal{obesities}\gdef\@journalfull{Obesities}\gdef\@journalshort{Obesities}\gdef\@doiabbr{obesities}\gdef\@ISSN{2673-4168}\gdef\@continuouspages{yes}}
\DeclareOption{oceans}{\gdef\@journal{oceans}\gdef\@journalfull{Oceans}\gdef\@journalshort{Oceans}\gdef\@doiabbr{oceans}\gdef\@ISSN{2673-1924}\gdef\@continuouspages{yes}}
\DeclareOption{ohbm}{\gdef\@journal{ohbm}\gdef\@journalfull{Journal of Otorhinolaryngology Hearing and Balance Medicine}\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}\gdef\@doiabbr{ohbm}\gdef\@ISSN{2504-463X}}
\DeclareOption{onco}{\gdef\@journal{onco}\gdef\@journalfull{Onco}\gdef\@journalshort{Onco}\gdef\@doiabbr{onco}\gdef\@ISSN{2673-7523}\gdef\@continuouspages{yes}}
%\DeclareOption{oncopathology}{\gdef\@journal{oncopathology}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{optics}{\gdef\@journal{optics}\gdef\@journalfull{Optics}\gdef\@journalshort{Optics}\gdef\@doiabbr{opt}\gdef\@ISSN{2673-3269}\gdef\@continuouspages{yes}}
\DeclareOption{oral}{\gdef\@journal{oral}\gdef\@journalfull{Oral}\gdef\@journalshort{Oral}\gdef\@doiabbr{oral}\gdef\@ISSN{2673-6373}\gdef\@continuouspages{yes}}
\DeclareOption{organics}{\gdef\@journal{organics}\gdef\@journalfull{Organics}\gdef\@journalshort{Organics}\gdef\@doiabbr{org}\gdef\@ISSN{2673-401X}\gdef\@continuouspages{yes}}
\DeclareOption{organoids}{\gdef\@journal{organoids}\gdef\@journalfull{Organoids}\gdef\@journalshort{Organoids}\gdef\@doiabbr{organoids}\gdef\@ISSN{2674-1172}\gdef\@continuouspages{yes}}
\DeclareOption{osteology}{\gdef\@journal{osteology}\gdef\@journalfull{Osteology}\gdef\@journalshort{Osteology}\gdef\@doiabbr{osteology}\gdef\@ISSN{2673-4036}\gdef\@continuouspages{yes}}
\DeclareOption{oxygen}{\gdef\@journal{oxygen}\gdef\@journalfull{Oxygen}\gdef\@journalshort{Oxygen}\gdef\@doiabbr{oxygen}\gdef\@ISSN{2673-9801}\gdef\@continuouspages{yes}}
\DeclareOption{parasites}{\gdef\@journal{parasites}\gdef\@journalfull{Parasites}\gdef\@journalshort{Parasites}\gdef\@doiabbr{parasites}\gdef\@ISSN{2673-5946}}
\DeclareOption{parasitologia}{\gdef\@journal{parasitologia}\gdef\@journalfull{Parasitologia}\gdef\@journalshort{Parasitologia}\gdef\@doiabbr{parasitologia}\gdef\@ISSN{2673-6772}\gdef\@continuouspages{yes}}
\DeclareOption{particles}{\gdef\@journal{particles}\gdef\@journalfull{Particles}\gdef\@journalshort{Particles}\gdef\@doiabbr{particles}\gdef\@ISSN{2571-712X}\gdef\@continuouspages{yes}}
\DeclareOption{pathogens}{\gdef\@journal{pathogens}\gdef\@journalfull{Pathogens}\gdef\@journalshort{Pathogens}\gdef\@doiabbr{pathogens}\gdef\@ISSN{2076-0817}}
\DeclareOption{pathophysiology}{\gdef\@journal{pathophysiology}\gdef\@journalfull{Pathophysiology}\gdef\@journalshort{Pathophysiology}\gdef\@doiabbr{pathophysiology}\gdef\@ISSN{0928-4680}\gdef\@continuouspages{yes}}
\DeclareOption{pediatrrep}{\gdef\@journal{pediatrrep}\gdef\@journalfull{Pediatric Reports}\gdef\@journalshort{Pediatr. Rep.}\gdef\@doiabbr{pediatric}\gdef\@ISSN{2036-7503}\gdef\@continuouspages{yes}}
\DeclareOption{pharmaceuticals}{\gdef\@journal{pharmaceuticals}\gdef\@journalfull{Pharmaceuticals}\gdef\@journalshort{Pharmaceuticals}\gdef\@doiabbr{ph}\gdef\@ISSN{1424-8247}}
\DeclareOption{pharmaceutics}{\gdef\@journal{pharmaceutics}\gdef\@journalfull{Pharmaceutics}\gdef\@journalshort{Pharmaceutics}\gdef\@doiabbr{pharmaceutics}\gdef\@ISSN{1999-4923}}
\DeclareOption{pharmacoepidemiology}{\gdef\@journal{pharmacoepidemiology}\gdef\@journalfull{Pharmacoepidemiology}\gdef\@journalshort{Pharmacoepidemiology}\gdef\@doiabbr{pharma}\gdef\@ISSN{2813-0618}\gdef\@continuouspages{yes}}
\DeclareOption{pharmacy}{\gdef\@journal{pharmacy}\gdef\@journalfull{Pharmacy}\gdef\@journalshort{Pharmacy}\gdef\@doiabbr{pharmacy}\gdef\@ISSN{2226-4787}}
\DeclareOption{philosophies}{\gdef\@journal{philosophies}\gdef\@journalfull{Philosophies}\gdef\@journalshort{Philosophies}\gdef\@doiabbr{philosophies}\gdef\@ISSN{2409-9287}}
\DeclareOption{photochem}{\gdef\@journal{photochem}\gdef\@journalfull{Photochem}\gdef\@journalshort{Photochem}\gdef\@doiabbr{photochem}\gdef\@ISSN{2673-7256}\gdef\@continuouspages{yes}}
\DeclareOption{photonics}{\gdef\@journal{photonics}\gdef\@journalfull{Photonics}\gdef\@journalshort{Photonics}\gdef\@doiabbr{photonics}\gdef\@ISSN{2304-6732}}
\DeclareOption{phycology}{\gdef\@journal{phycology}\gdef\@journalfull{Phycology}\gdef\@journalshort{Phycology}\gdef\@doiabbr{phycology}\gdef\@ISSN{2673-9410}\gdef\@continuouspages{yes}}
\DeclareOption{physchem}{\gdef\@journal{physchem}\gdef\@journalfull{Physchem}\gdef\@journalshort{Physchem}\gdef\@doiabbr{physchem}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{physics}{\gdef\@journal{physics}\gdef\@journalfull{Physics}\gdef\@journalshort{Physics}\gdef\@doiabbr{physics}\gdef\@ISSN{2624-8174}\gdef\@continuouspages{yes}}
\DeclareOption{physiologia}{\gdef\@journal{physiologia}\gdef\@journalfull{Physiologia}\gdef\@journalshort{Physiologia}\gdef\@doiabbr{physiologia}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{plants}{\gdef\@journal{plants}\gdef\@journalfull{Plants}\gdef\@journalshort{Plants}\gdef\@doiabbr{plants}\gdef\@ISSN{2223-7747}}
\DeclareOption{plasma}{\gdef\@journal{plasma}\gdef\@journalfull{Plasma}\gdef\@journalshort{Plasma}\gdef\@doiabbr{plasma}\gdef\@ISSN{2571-6182}\gdef\@continuouspages{yes}}
\DeclareOption{pollutants}{\gdef\@journal{pollutants}\gdef\@journalfull{Pollutants}\gdef\@journalshort{Pollutants}\gdef\@doiabbr{pollutants}\gdef\@ISSN{2673-4672}\gdef\@continuouspages{yes}}
\DeclareOption{polymers}{\gdef\@journal{polymers}\gdef\@journalfull{Polymers}\gdef\@journalshort{Polymers}\gdef\@doiabbr{polym}\gdef\@ISSN{2073-4360}}
\DeclareOption{polysaccharides}{\gdef\@journal{polysaccharides}\gdef\@journalfull{Polysaccharides}\gdef\@journalshort{Polysaccharides}\gdef\@doiabbr{polysaccharides}\gdef\@ISSN{2673-4176}\gdef\@continuouspages{yes}}
\DeclareOption{poultry}{\gdef\@journal{poultry}\gdef\@journalfull{Poultry}\gdef\@journalshort{Poultry}\gdef\@doiabbr{poultry}\gdef\@ISSN{2674-1164}\gdef\@continuouspages{yes}}
\DeclareOption{powders}{\gdef\@journal{powders}\gdef\@journalfull{Powders}\gdef\@journalshort{Powders}\gdef\@doiabbr{powders}\gdef\@ISSN{2674-0516}\gdef\@continuouspages{yes}}
\DeclareOption{preprints}{\gdef\@journal{preprints}\gdef\@journalfull{Preprints}\gdef\@journalshort{Preprints}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{proceedings}{\gdef\@journal{proceedings}\gdef\@journalfull{Proceedings}\gdef\@journalshort{Proceedings}\gdef\@doiabbr{proceedings}\gdef\@ISSN{2504-3900}}
\DeclareOption{processes}{\gdef\@journal{processes}\gdef\@journalfull{Processes}\gdef\@journalshort{Processes}\gdef\@doiabbr{pr}\gdef\@ISSN{2227-9717}}
\DeclareOption{prosthesis}{\gdef\@journal{prosthesis}\gdef\@journalfull{Prosthesis}\gdef\@journalshort{Prosthesis}\gdef\@doiabbr{prosthesis}\gdef\@ISSN{2673-1592}\gdef\@continuouspages{yes}}
\DeclareOption{proteomes}{\gdef\@journal{proteomes}\gdef\@journalfull{Proteomes}\gdef\@journalshort{Proteomes}\gdef\@doiabbr{proteomes}\gdef\@ISSN{2227-7382}}
\DeclareOption{psf}{\gdef\@journal{psf}\gdef\@journalfull{Physical Sciences Forum}\gdef\@journalshort{Phys. Sci. Forum}\gdef\@doiabbr{psf}\gdef\@ISSN{2673-9984}}
\DeclareOption{psych}{\gdef\@journal{psych}\gdef\@journalfull{Psych}\gdef\@journalshort{Psych}\gdef\@doiabbr{psych}\gdef\@ISSN{2624-8611}\gdef\@continuouspages{yes}}
\DeclareOption{psychiatryint}{\gdef\@journal{psychiatryint}\gdef\@journalfull{Psychiatry International}\gdef\@journalshort{Psychiatry Int.}\gdef\@doiabbr{psychiatryint}\gdef\@ISSN{2673-5318}\gdef\@continuouspages{yes}}
\DeclareOption{psychoactives}{\gdef\@journal{psychoactives}\gdef\@journalfull{Psychoactives}\gdef\@journalshort{Psychoactives}\gdef\@doiabbr{psychoactives}\gdef\@ISSN{2813-1851}\gdef\@continuouspages{yes}}
\DeclareOption{publications}{\gdef\@journal{publications}\gdef\@journalfull{Publications}\gdef\@journalshort{Publications}\gdef\@doiabbr{publications}\gdef\@ISSN{2304-6775}}
\DeclareOption{quantumrep}{\gdef\@journal{quantumrep}\gdef\@journalfull{Quantum Reports}\gdef\@journalshort{Quantum Rep.}\gdef\@doiabbr{quantum}\gdef\@ISSN{2624-960X}\gdef\@continuouspages{yes}}
\DeclareOption{quaternary}{\gdef\@journal{quaternary}\gdef\@journalfull{Quaternary}\gdef\@journalshort{Quaternary}\gdef\@doiabbr{quat}\gdef\@ISSN{2571-550X}}
\DeclareOption{qubs}{\gdef\@journal{qubs}\gdef\@journalfull{Quantum Beam Science}\gdef\@journalshort{Quantum Beam Sci.}\gdef\@doiabbr{qubs}\gdef\@ISSN{2412-382X}}
\DeclareOption{radiation}{\gdef\@journal{radiation}\gdef\@journalfull{Radiation}\gdef\@journalshort{Radiation}\gdef\@doiabbr{radiation}\gdef\@ISSN{2673-592X}\gdef\@continuouspages{yes}}
\DeclareOption{reactions}{\gdef\@journal{reactions}\gdef\@journalfull{Reactions}\gdef\@journalshort{Reactions}\gdef\@doiabbr{reactions}\gdef\@ISSN{2624-781X}\gdef\@continuouspages{yes}}
\DeclareOption{receptors}{\gdef\@journal{receptors}\gdef\@journalfull{Receptors}\gdef\@journalshort{Receptors}\gdef\@doiabbr{receptors}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{recycling}{\gdef\@journal{recycling}\gdef\@journalfull{Recycling}\gdef\@journalshort{Recycling}\gdef\@doiabbr{recycling}\gdef\@ISSN{2313-4321}}
\DeclareOption{regeneration}{\gdef\@journal{regeneration}\gdef\@journalfull{Regeneration}\gdef\@journalshort{Regeneration}\gdef\@doiabbr{regeneration}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{religions}{\gdef\@journal{religions}\gdef\@journalfull{Religions}\gdef\@journalshort{Religions}\gdef\@doiabbr{rel}\gdef\@ISSN{2077-1444}}
\DeclareOption{remotesensing}{\gdef\@journal{remotesensing}\gdef\@journalfull{Remote Sensing}\gdef\@journalshort{Remote Sens.}\gdef\@doiabbr{rs}\gdef\@ISSN{2072-4292}}
\DeclareOption{reports}{\gdef\@journal{reports}\gdef\@journalfull{Reports}\gdef\@journalshort{Reports}\gdef\@doiabbr{reports}\gdef\@ISSN{2571-841X}}
\DeclareOption{reprodmed}{\gdef\@journal{reprodmed}\gdef\@journalfull{Reproductive Medicine}\gdef\@journalshort{Reprod. Med.}\gdef\@doiabbr{reprodmed}\gdef\@ISSN{2673-3897}\gdef\@continuouspages{yes}}
\DeclareOption{resources}{\gdef\@journal{resources}\gdef\@journalfull{Resources}\gdef\@journalshort{Resources}\gdef\@doiabbr{resources}\gdef\@ISSN{2079-9276}}
\DeclareOption{rheumato}{\gdef\@journal{rheumato}\gdef\@journalfull{Rheumato}\gdef\@journalshort{Rheumato}\gdef\@doiabbr{rheumato}\gdef\@ISSN{2674-0621}\gdef\@continuouspages{yes}}
\DeclareOption{risks}{\gdef\@journal{risks}\gdef\@journalfull{Risks}\gdef\@journalshort{Risks}\gdef\@doiabbr{risks}\gdef\@ISSN{2227-9091}}
\DeclareOption{robotics}{\gdef\@journal{robotics}\gdef\@journalfull{Robotics}\gdef\@journalshort{Robotics}\gdef\@doiabbr{robotics}\gdef\@ISSN{2218-6581}}
\DeclareOption{ruminants}{\gdef\@journal{ruminants}\gdef\@journalfull{Ruminants}\gdef\@journalshort{Ruminants}\gdef\@doiabbr{ruminants}\gdef\@ISSN{2673-933X}\gdef\@continuouspages{yes}}
\DeclareOption{safety}{\gdef\@journal{safety}\gdef\@journalfull{Safety}\gdef\@journalshort{Safety}\gdef\@doiabbr{safety}\gdef\@ISSN{2313-576X}}
\DeclareOption{sci}{\gdef\@journal{sci}\gdef\@journalfull{Sci}\gdef\@journalshort{Sci}\gdef\@doiabbr{sci}\gdef\@ISSN{2413-4155}}
\DeclareOption{scipharm}{\gdef\@journal{scipharm}\gdef\@journalfull{Scientia Pharmaceutica}\gdef\@journalshort{Sci. Pharm.}\gdef\@doiabbr{scipharm}\gdef\@ISSN{2218-0532}}
\DeclareOption{seeds}{\gdef\@journal{seeds}\gdef\@journalfull{Seeds}\gdef\@journalshort{Seeds}\gdef\@doiabbr{seeds}\gdef\@ISSN{2674-1024}\gdef\@continuouspages{yes}}
\DeclareOption{sensors}{\gdef\@journal{sensors}\gdef\@journalfull{Sensors}\gdef\@journalshort{Sensors}\gdef\@doiabbr{s}\gdef\@ISSN{1424-8220}}
\DeclareOption{separations}{\gdef\@journal{separations}\gdef\@journalfull{Separations}\gdef\@journalshort{Separations}\gdef\@doiabbr{separations}\gdef\@ISSN{2297-8739}}
\DeclareOption{sexes}{\gdef\@journal{sexes}\gdef\@journalfull{Sexes}\gdef\@journalshort{Sexes}\gdef\@doiabbr{sexes}\gdef\@ISSN{2411-5118}\gdef\@continuouspages{yes}}
\DeclareOption{signals}{\gdef\@journal{signals}\gdef\@journalfull{Signals}\gdef\@journalshort{Signals}\gdef\@doiabbr{signals}\gdef\@ISSN{2624-6120}\gdef\@continuouspages{yes}}
\DeclareOption{sinusitis}{\gdef\@journal{sinusitis}\gdef\@journalfull{Sinusitis}\gdef\@journalshort{Sinusitis}\gdef\@doiabbr{sinusitis}\gdef\@ISSN{2309-107X}\gdef\@continuouspages{yes}}
\DeclareOption{skins}{\gdef\@journal{skins}\gdef\@journalfull{Skins}\gdef\@journalshort{Skins}\gdef\@doiabbr{skins}\gdef\@ISSN{}}
\DeclareOption{smartcities}{\gdef\@journal{smartcities}\gdef\@journalfull{Smart Cities}\gdef\@journalshort{Smart Cities}\gdef\@doiabbr{smartcities}\gdef\@ISSN{2624-6511}\gdef\@continuouspages{yes}}
\DeclareOption{sna}{\gdef\@journal{sna}\gdef\@journalfull{Sinusitis and Asthma}\gdef\@journalshort{Sinusitis Asthma}\gdef\@doiabbr{sna}\gdef\@ISSN{2624-7003}}
\DeclareOption{societies}{\gdef\@journal{societies}\gdef\@journalfull{Societies}\gdef\@journalshort{Societies}\gdef\@doiabbr{soc}\gdef\@ISSN{2075-4698}}
\DeclareOption{socsci}{\gdef\@journal{socsci}\gdef\@journalfull{Social Sciences}\gdef\@journalshort{Soc. Sci.}\gdef\@doiabbr{socsci}\gdef\@ISSN{2076-0760}}
\DeclareOption{software}{\gdef\@journal{software}\gdef\@journalfull{Software}\gdef\@journalshort{Software}\gdef\@doiabbr{software}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{soilsystems}{\gdef\@journal{soilsystems}\gdef\@journalfull{Soil Systems}\gdef\@journalshort{Soil Syst.}\gdef\@doiabbr{soilsystems}\gdef\@ISSN{2571-8789}}
\DeclareOption{solar}{\gdef\@journal{solar}\gdef\@journalfull{Solar}\gdef\@journalshort{Solar}\gdef\@doiabbr{solar}\gdef\@ISSN{2673-9941}\gdef\@continuouspages{yes}}
\DeclareOption{solids}{\gdef\@journal{solids}\gdef\@journalfull{Solids}\gdef\@journalshort{Solids}\gdef\@doiabbr{solids}\gdef\@ISSN{2673-6497}\gdef\@continuouspages{yes}}
\DeclareOption{spectroscj}{\gdef\@journal{spectroscj}\gdef\@journalfull{Spectroscopy Journal}\gdef\@journalshort{Spectrosc. J.}\gdef\@doiabbr{spectroscj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{sports}{\gdef\@journal{sports}\gdef\@journalfull{Sports}\gdef\@journalshort{Sports}\gdef\@doiabbr{sports}\gdef\@ISSN{2075-4663}}
\DeclareOption{standards}{\gdef\@journal{standards}\gdef\@journalfull{Standards}\gdef\@journalshort{Standards}\gdef\@doiabbr{standards}\gdef\@ISSN{2305-6703}\gdef\@continuouspages{yes}}
\DeclareOption{stats}{\gdef\@journal{stats}\gdef\@journalfull{Stats}\gdef\@journalshort{Stats}\gdef\@doiabbr{stats}\gdef\@ISSN{2571-905X}\gdef\@continuouspages{yes}}
\DeclareOption{std}{\gdef\@journal{std}\gdef\@journalfull{Surgical Techniques Development}\gdef\@journalshort{Surg. Tech. Dev.}\gdef\@doiabbr{std}\gdef\@ISSN{2038-9582}\gdef\@continuouspages{yes}}
\DeclareOption{stresses}{\gdef\@journal{stresses}\gdef\@journalfull{Stresses}\gdef\@journalshort{Stresses}\gdef\@doiabbr{stresses}\gdef\@ISSN{2673-7140}\gdef\@continuouspages{yes}}
\DeclareOption{surfaces}{\gdef\@journal{surfaces}\gdef\@journalfull{Surfaces}\gdef\@journalshort{Surfaces}\gdef\@doiabbr{surfaces}\gdef\@ISSN{2571-9637}\gdef\@continuouspages{yes}}
\DeclareOption{surgeries}{\gdef\@journal{surgeries}\gdef\@journalfull{Surgeries}\gdef\@journalshort{Surgeries}\gdef\@doiabbr{surgeries}\gdef\@ISSN{2017-2017}\gdef\@continuouspages{yes}}
\DeclareOption{suschem}{\gdef\@journal{suschem}\gdef\@journalfull{Sustainable Chemistry}\gdef\@journalshort{Sustain. Chem.}\gdef\@doiabbr{suschem}\gdef\@ISSN{2673-4079}\gdef\@continuouspages{yes}}
\DeclareOption{sustainability}{\gdef\@journal{sustainability}\gdef\@journalfull{Sustainability}\gdef\@journalshort{Sustainability}\gdef\@doiabbr{su}\gdef\@ISSN{2071-1050}}
\DeclareOption{symmetry}{\gdef\@journal{symmetry}\gdef\@journalfull{Symmetry}\gdef\@journalshort{Symmetry}\gdef\@doiabbr{sym}\gdef\@ISSN{2073-8994}}
\DeclareOption{synbio}{\gdef\@journal{synbio}\gdef\@journalfull{Synbio}\gdef\@journalshort{Synbio}\gdef\@doiabbr{synbio}\gdef\@ISSN{2674-0583}\gdef\@continuouspages{yes}}
\DeclareOption{systems}{\gdef\@journal{systems}\gdef\@journalfull{Systems}\gdef\@journalshort{Systems}\gdef\@doiabbr{systems}\gdef\@ISSN{2079-8954}}
\DeclareOption{taxonomy}{\gdef\@journal{taxonomy}\gdef\@journalfull{Taxonomy}\gdef\@journalshort{Taxonomy}\gdef\@doiabbr{taxonomy}\gdef\@ISSN{2673-6500}\gdef\@continuouspages{yes}}
\DeclareOption{technologies}{\gdef\@journal{technologies}\gdef\@journalfull{Technologies}\gdef\@journalshort{Technologies}\gdef\@doiabbr{technologies}\gdef\@ISSN{2227-7080}}
\DeclareOption{telecom}{\gdef\@journal{telecom}\gdef\@journalfull{Telecom}\gdef\@journalshort{Telecom}\gdef\@doiabbr{telecom}\gdef\@ISSN{2673-4001}\gdef\@continuouspages{yes}}
\DeclareOption{test}{\gdef\@journal{test}\gdef\@journalfull{Test}\gdef\@journalshort{Test}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{textiles}{\gdef\@journal{textiles}\gdef\@journalfull{Textiles}\gdef\@journalshort{Textiles}\gdef\@doiabbr{textiles}\gdef\@ISSN{2673-7248}\gdef\@continuouspages{yes}}
\DeclareOption{thalassrep}{\gdef\@journal{thalassrep}\gdef\@journalfull{Thalassemia Reports}\gdef\@journalshort{Thalass. Rep.}\gdef\@doiabbr{thalassrep}\gdef\@ISSN{2039-4365}\gdef\@continuouspages{yes}}
\DeclareOption{thermo}{\gdef\@journal{thermo}\gdef\@journalfull{Thermo}\gdef\@journalshort{Thermo}\gdef\@doiabbr{thermo}\gdef\@ISSN{2673-7264}\gdef\@continuouspages{yes}}
\DeclareOption{tomography}{\gdef\@journal{tomography}\gdef\@journalfull{Tomography}\gdef\@journalshort{Tomography}\gdef\@doiabbr{tomography}\gdef\@ISSN{2379-139X}\gdef\@continuouspages{yes}}
\DeclareOption{tourismhosp}{\gdef\@journal{tourismhosp}\gdef\@journalfull{Tourism and Hospitality}\gdef\@journalshort{Tour. Hosp.}\gdef\@doiabbr{tourhosp}\gdef\@ISSN{2673-5768}\gdef\@continuouspages{yes}}
\DeclareOption{toxics}{\gdef\@journal{toxics}\gdef\@journalfull{Toxics}\gdef\@journalshort{Toxics}\gdef\@doiabbr{toxics}\gdef\@ISSN{2305-6304}}
\DeclareOption{toxins}{\gdef\@journal{toxins}\gdef\@journalfull{Toxins}\gdef\@journalshort{Toxins}\gdef\@doiabbr{toxins}\gdef\@ISSN{2072-6651}}
\DeclareOption{transplantology}{\gdef\@journal{transplantology}\gdef\@journalfull{Transplantology}\gdef\@journalshort{Transplantology}\gdef\@doiabbr{transplantology}\gdef\@ISSN{2673-3943}\gdef\@continuouspages{yes}}
\DeclareOption{transportation}{\gdef\@journal{transportation}\gdef\@journalfull{Transportation}\gdef\@journalshort{Transportation}\gdef\@doiabbr{transportation}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{traumacare}{\gdef\@journal{traumacare}\gdef\@journalfull{Trauma Care}\gdef\@journalshort{Trauma Care}\gdef\@doiabbr{traumacare}\gdef\@ISSN{2673-866X}\gdef\@continuouspages{yes}}
\DeclareOption{traumas}{\gdef\@journal{traumas}\gdef\@journalfull{Traumas}\gdef\@journalshort{Traumas}\gdef\@doiabbr{traumas}\gdef\@ISSN{2673-7477}\gdef\@continuouspages{yes}}
\DeclareOption{tropicalmed}{\gdef\@journal{tropicalmed}\gdef\@journalfull{Tropical Medicine and Infectious Disease}\gdef\@journalshort{Trop. Med. Infect. Dis.}\gdef\@doiabbr{tropicalmed}\gdef\@ISSN{2414-6366}}
\DeclareOption{universe}{\gdef\@journal{universe}\gdef\@journalfull{Universe}\gdef\@journalshort{Universe}\gdef\@doiabbr{universe}\gdef\@ISSN{2218-1997}}
\DeclareOption{urbansci}{\gdef\@journal{urbansci}\gdef\@journalfull{Urban Science}\gdef\@journalshort{Urban Sci.}\gdef\@doiabbr{urbansci}\gdef\@ISSN{2413-8851}}
\DeclareOption{uro}{\gdef\@journal{uro}\gdef\@journalfull{Uro}\gdef\@journalshort{Uro}\gdef\@doiabbr{uro}\gdef\@ISSN{2673-4397}\gdef\@continuouspages{yes}}
\DeclareOption{vaccines}{\gdef\@journal{vaccines}\gdef\@journalfull{Vaccines}\gdef\@journalshort{Vaccines}\gdef\@doiabbr{vaccines}\gdef\@ISSN{2076-393X}}
\DeclareOption{vehicles}{\gdef\@journal{vehicles}\gdef\@journalfull{Vehicles}\gdef\@journalshort{Vehicles}\gdef\@doiabbr{vehicles}\gdef\@ISSN{2624-8921}\gdef\@continuouspages{yes}}
\DeclareOption{venereology}{\gdef\@journal{venereology}\gdef\@journalfull{Venereology}\gdef\@journalshort{Venereology}\gdef\@doiabbr{venereology}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{vetsci}{\gdef\@journal{vetsci}\gdef\@journalfull{Veterinary Sciences}\gdef\@journalshort{Vet. Sci.}\gdef\@doiabbr{vetsci}\gdef\@ISSN{2306-7381}}
\DeclareOption{vibration}{\gdef\@journal{vibration}\gdef\@journalfull{Vibration}\gdef\@journalshort{Vibration}\gdef\@doiabbr{vibration}\gdef\@ISSN{2571-631X}\gdef\@continuouspages{yes}}
\DeclareOption{virtualworlds}{\gdef\@journal{virtualworlds}\gdef\@journalfull{Virtual Worlds}\gdef\@journalshort{Virtual Worlds}\gdef\@doiabbr{virtualworlds}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{viruses}{\gdef\@journal{viruses}\gdef\@journalfull{Viruses}\gdef\@journalshort{Viruses}\gdef\@doiabbr{v}\gdef\@ISSN{1999-4915}}
\DeclareOption{vision}{\gdef\@journal{vision}\gdef\@journalfull{Vision}\gdef\@journalshort{Vision}\gdef\@doiabbr{vision}\gdef\@ISSN{2411-5150}}
\DeclareOption{waste}{\gdef\@journal{waste}\gdef\@journalfull{Waste}\gdef\@journalshort{Waste}\gdef\@doiabbr{waste}\gdef\@ISSN{2813-0391}\gdef\@continuouspages{yes}}
\DeclareOption{water}{\gdef\@journal{water}\gdef\@journalfull{Water}\gdef\@journalshort{Water}\gdef\@doiabbr{w}\gdef\@ISSN{2073-4441}}
\DeclareOption{wem}{\gdef\@journal{wem}\gdef\@journalfull{Wildlife Ecology and Management}\gdef\@journalshort{Wildl. Ecol. Manag.}\gdef\@doiabbr{}\gdef\@ISSN{1234-4321}}
\DeclareOption{wevj}{\gdef\@journal{wevj}\gdef\@journalfull{World Electric Vehicle Journal}\gdef\@journalshort{World Electr. Veh. J.}\gdef\@doiabbr{wevj}\gdef\@ISSN{2032-6653}}
\DeclareOption{wind}{\gdef\@journal{wind}\gdef\@journalfull{Wind}\gdef\@journalshort{Wind}\gdef\@doiabbr{wind}\gdef\@ISSN{2674-032X}\gdef\@continuouspages{yes}}
\DeclareOption{women}{\gdef\@journal{women}\gdef\@journalfull{Women}\gdef\@journalshort{Women}\gdef\@doiabbr{women}\gdef\@ISSN{2673-4184}\gdef\@continuouspages{yes}}
\DeclareOption{world}{\gdef\@journal{world}\gdef\@journalfull{World}\gdef\@journalshort{World}\gdef\@doiabbr{world}\gdef\@ISSN{2673-4060}\gdef\@continuouspages{yes}}
\DeclareOption{youth}{\gdef\@journal{youth}\gdef\@journalfull{Youth}\gdef\@journalshort{Youth}\gdef\@doiabbr{youth}\gdef\@ISSN{2673-995X}\gdef\@continuouspages{yes}}
\DeclareOption{zoonoticdis}{\gdef\@journal{zoonoticdis}\gdef\@journalfull{Zoonotic Diseases}\gdef\@journalshort{Zoonotic Dis.}\gdef\@doiabbr{zoonoticdis}\gdef\@ISSN{2813-0227}\gdef\@continuouspages{yes}}


==> paper/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

It is undeniable that advancements in \textit{Search Engines (SE)}~\cite{croft2010search} represent a revolution without precedent in human history for information dissemination. Due to the large amount of readily available data, knowing how to construct \textit{Search Queries (SQs)}~\cite{sqsdef} has become a fundamental skill. From Google~\cite{google} to Wikipedia~\cite{wikipedia}, most SEs require users to type a text-based search query to retrieve relevant information. Although much data is available through such SEs, most of the structured datasets, such as the UNData~\cite{undata} time-series world indicators, live outside their scope and cannot be incorporated into search queries. On the other hand, the information contained in structured datasets is typically available to probe through visualization tools or interfaces. One example is Gapminder~\cite{rosling2012gapminderorg}, where users can visualize animated charts displaying the UNData dataset. Despite their popularity, no individual visualization tool comes close to the sheer amount of information available through Wikipedia's hyperlinked text documents. Therefore, even if one uses, for instance, Gapminder to discover global misconceptions~\cite{sarma2017hans}, they will undeniably be required to search elsewhere for extra information regarding the underlying findings.

The task of generating text-based SQs for SEs is, broadly speaking, done by the users themselves. However, this process can be challenging since the translation between user intent and keywords is sometimes not trivial, causing users not to find the information being looked for~\cite{kammerer2012children}. Beyond regular keyword lists, other search strategies are available to address such limitations. For instance, it is also possible to ``search by image''~\cite{reilly2017reverse}, where users can find images similar to a given image, or ``search by natural language''~\cite{cafarella2005search, kammerer2012children}, where users can search using descriptive texts. 

However, when considering structured datasets, up to our knowledge, there is no mechanism to use pieces of visual data, such as user selections in a line chart, to search for related information using general-purpose SEs. Instead of using visual selections, there are solutions that either use visualizations as outputs~\cite{hullman2013contextifier, badam2018elastic, yu2019flowsense} or as a visual interface to manually construct what is essentially a text-based query~\cite{kraska2018northstar, zhou2021modeling, borland2019selection, borland2020selection}. Even though such visualizations are shown to aid the information gathering processes, in these works, the use of visual selections as \textit{visual search queries} to fetch relevant information from general-purpose SEs is an unexplored concept. Also, various examples of search query suggestions for data analysis~\cite{ooi2015survey, yi2017autog} have been proposed, but the use of such techniques applied to \textit{visual search queries} during data analysis is similarly unexplored.

This paper proposes \textit{QuEry for visual Data Analysis (Q4EDA)}, a novel framework that converts user visual selections to relevant search queries to be used for general purposes search engines, like Google or Wikipedia. 
%
Using query expansion and suggestion techniques, one of the promising applications for Q4EDA is to allow users to perform an enhanced visual analysis of time-series dataset collections. To use Q4EDA in this context, a visualization tool, such as Gapminder or Tableau~\cite{zhang2012visual} captures and forwards user \textit{visual selection queries (VQs)} to Q4EDA, then Q4EDA processes the selection and outputs an SQ which can then be used on general-purpose SEs. Q4EDA also suggests other potential time series related to the selected event within the dataset collection to be subsequently investigated. In summary, the main contributions of this paper are:

\squishlist 
\item A conversion technique to transform visual selection queries into valid and stable search queries usable in general-purpose search engines; 

\item A strategy to expand the converted search query to better retrieve related text documents and provide suggestion ranking lists with data related to the visual selection query;

\item An exploratory data analysis application example that uses Q4EDA in practice to provide means to find more (textual) information related to an observed pattern compared to the standard manual keyword-based queries.
\squishend

%FVP.: acho que isso nao precisa
%Although Q4EDA expects the VQ to match a particular specification, there are no strict conditions of what visual metaphor is being used to generate the VQ as long as the required data is provided. 
%
%Likewise, Q4EDA also provides flexibility in its output which is only dependent on the implemented SE formatters. Therefore, Q4EDA's two-stage conversion process allows for multiple inputs and outputs specifications to be implemented depending on their usage. 
%

%
%FVP.: isso tem cara de conclusao
%In this paper, we limited Q4EDA's input specification to time-series dataset collections, such as UNData~\cite{undata}, and its output to Elasticsearch simple-queries~\cite{SimpleElastic} which, in conjunction with Wikipedia~\cite{cirrussearch}, can be used for information retrieval of visual selection queries. That said, Q4EDA's modular nature readily accepts modifications for many other application possibilities.

The remainder of the paper is structured as follows. In Sec.~\ref{sec:related}, we discuss related work involving techniques that seek to interpret visual interactivity as queries and how they execute and use the results of their query. In Sec.~\ref{sec:method}, we formalize the problem and outline the Q4EDA solution. In Sec.~\ref{sec:results}, we present use-case examples of how visualization tools can use Q4EDA. Evaluations through user survey and query stability performance are then presented in Sec.~\ref{sec:usereval}, indicating a good degree of stability and reproducibility of the search queries and overall success of Q4EDA in enhancing users' ability to probe for relevant information of patterns or events found during visual data analysis. Finally, in Sec.~\ref{sec:limitations} we discuss Q4EDA limitations and in Sec.~\ref{sec:conclusions} we draw our conclusions.









%%%%%%%%%%%%%
% ter certeza que discutimos IR bem em analise de dados estruturados
% colocar tb aqui coisa q eu coloquei no use-case, em que o nosso uso e que o q4eda nao faz a viz, mas espera que alguem faz a viz e que por uma selecao na viz, agente faz a conversao e suggestion (deixa suggestion pro fim e conversao primeiro)
% possivel uso do nome: q4eda usa dados estruturados
% novo rumo: precisa falar que temps uma interface grafica (pq a conferencia pede) em que o usuario seleciona qual dados ele quer pesquisar
%LC: revisar se.. tem que falar o que existe na literatura que faz busca usando dados estruturados e que faltou alguma coisa em relacao a query suggestion
%
%
%Within \textit{Visual Analytics (VA)} we also find that during \textit{Exploratory Data Analysis}, there are tools that not just allow for regular selections through lists and checkboxes, like Gapminder~\cite{rosling2012gapminderorg}, but many also allow for \textit{visual selections}, such as box-select within a scatter-plot, in order to interactively perform analysis~\cite{kraska2018northstar, zhou2021modeling}. Although such interactions are used for great effectiveness to perform data filtering or data selection, there is no VA framework which uses such selection as a means to construct a search query for general purpose SEs.


%In evaluating this work, we focused in testing weather Q4EDA performs better than asking users to manually convert visual insights into search queries. This is validated by analysing users' answers when using Q4EDA's automatic conversion versus manually searching Wikipedia about certain visual patterns of interest found in line-charts of world demographics indicators. 
%
%FVP: so falaria das conclusoes da avalicao, nao dela em si.
% LC: TODO: acrecentar a ideia que vamos limitar pra 2 niveis de metadado

==> paper/2_related.tex <==
\section{Related Work}
\label{sec:related}

In order to support users in visual data analysis, some tools and techniques allow for a non-obstructive exploratory approach through visual interactivity~\cite{srinivasan2018augmenting, kraska2018northstar}, among the most relevant is NorthStar~\cite{kraska2018northstar}, which goes in-depth into the difficulties of providing an exploratory system that follows responsive and real-time guidelines for intuitive and engaging user exploratory analysis while at the same time utilizing automatic problem detectors throughout the entire workflow to reduce the amount of potential bias or incorrect insights generated through the exploration. However, although a certain level of ``query conversion'' is done through these tools or techniques, they still expect what is essentially a text-based query to be constructed manually through their visual interface. Furthermore, these tools use the query to retrieve data from domain-specific databases, which differs from our proposed query conversion method for search engines. Moreover, although research has identified other ways to encode visual findings and hypotheses beyond visual query constructors~\cite{suh2022grammar}, no existing work, as far as the authors know, has demonstrated ways to use such methodology to convert a visual selection into a search query as Q4EDA proposes.

Considering the perspective of visual selection queries and its related information from external datasets, some approaches focus on extracting or generating automatic visualizations and annotations. Despite representing significant progress, the amount of analysis enhancement they provide is limited to the generation of visual metaphors~\cite{cui2019text, lin2018vizbywiki, bryan2016temporal} and of visual feature extractions~\cite{bryan2016temporal, tang2017extracting, ding2019quickinsights} produced from a single dataset used for analysis. Other works focus on generating enhanced visualizations by displaying one dataset as a visual feature of the other. These visual features can be annotations~\cite{hullman2013contextifier, kwon2014visjockey}, can involve textual queries to generate visualizations~\cite{yu2019flowsense, luo2018deepeye, metoyer2018coupling, hoque2017applying}, can define a question-answer interface to visualizations~\cite{kim2020answering, kafle2020answering, yu2020cross}, can use textual datasets to help the understandability of structured datasets~\cite{badam2018elastic, kim2018facilitating, yu2019flowsense, srinivasan2017orko}, or can automatic link text to images for use within visualizations~\cite{mogadala2019trends, yu2020reasoning, dhelim2020compath}. The research has shown approachable and engaging ways to optimize visualizations and analysis by using text-based datasets and NLP techniques. \obs{Of them, usage of heterogeneous data~\cite{dhelim2020compath} an cross-modal methods~\cite{yu2020reasoning, yu2020cross} has shown that utilizing multimodal datasets, such as time-series and text, provides significant advantages to the user's analysis.} Although many of them use some query to retrieve information from text, no one uses external search engines as the target of such queries. Instead, they focus on specific text datasets. These efforts show a focus on analyzing a single dataset with the aid of another, which provides NLP capabilities during analysis. However, such approaches differ from the proposal of Q4EDA where we do not just convert visual search queries and provide valid search queries to be used in existing search engines but also provide query suggestions, aiding the analysis in many ways. 

Visual Analytics has also recently started to use heterogeneous datasets for analysis, and one such work done by~\citet{zhou2021modeling} proposes a method of using users' interactions to quantify their attention and, from it, decide which medical documents to present to the user. Arguably similar to Q4EDA, \citet{zhou2021modeling} uses a textual database and a query system from their previous work Cadence~\cite{borland2019selection, borland2020selection}. Although their text database does not significantly differ from existing search engines, hence approaching Q4EDA's proposal, this work does not provide an actual query conversion process, nor proposes methods of query suggestions, nor allows for visual selections as queries. Instead, queries are again constructed manually using the Cadence system through a drag-and-drop interface to perform the search. This procedure is arguably most similar to the interface of NorthStar~\cite{kraska2018northstar} as opposed to Q4EDA.

Significant effort has been made by the information retrieval community to propose better ways to use search engines during data analysis. The practice of retrieving information~\cite{croft2010search} describes ways to expand a query, so its effectiveness is more relevant to users when executed in a SE~\cite{zhang2009concept, carpineto2012survey, azad2019query, dahir2021query} and how to provide suggestions for future queries~\cite{ooi2015survey}. Although their techniques are very relevant to Q4EDA, the vast majority are non-visual approaches that describe advances in how to perform query expansion of a keyword or natural language search query as opposed to Q4EDA's \textit{visual selection queries}. Among the ones that use visualizations, they either use it only to display information, lacking interactivity~\cite{hoeber2005visualization}, or use it as a query builder interface, where there is no concept of visual selection queries~\cite{khazaei2017supporting}, focuses on visualizing a manually or interactively constructed query~\cite{scells2018searchrefiner, russell20182dsearch}. Indeed, the authors are not aware of any research within the information retrieval community which transforms or converts visual selections into SQ automatically, that is, without any user intervention to manually, even if through visual interfaces, construct the search query. Q4EDA aims to fill this gap where users are not required to interpret the available data and manually construct the search query. Instead, users can visually select portions of existing visualizations, and the selection is automatically converted into a valid search query for use in search engines.

Both information retrieval and the data management communities have had great strides in connecting heterogeneous data, such as time-series datasets and text documents. Currently, one of the major advances in this direction is the concept of dataspaces~\cite{curry2020dataspaces, franklin2005databases} and knowledge graphs~\cite{dahir2021query, balalau2020graph, martinez2015automated, auer2007dbpedia, yi2017autog}. Manual, semi-automatic, and automatic procedures for matching and linking these have been studied~\cite{golshan2017data, mountantonakis2019large, mogadala2019trends, arya2021survey, christophides2019end, groger2014deep, roy2005towards}. 
Though some contributions links structured datasets within visualizations to external data and others link data to text documents, no related work performs the full path from visual selections to search engine responses as far as the authors are aware. Though Q4EDA uses many of the concepts shared among these valuable contributions, Q4EDA blurs the line between visual interaction, database query, and information retrieval to deliver what it proposes.

In summary, existing works provide many relevant works which use textual datasets to enhance data analysis, but they provide no \textit{visual selection query} conversion capabilities. Many do not support search engines nor provide query suggestions from text documents extracted from said search engine. Some newer work exemplifies the benefits of linking structured datasets to textual counterparts for data analysis enhancement. However, they still fail to provide a way for users to analyze datasets through visual selection queries, such as a box selection within a line chart, and simultaneously be provided suggestions of said visual selection. Instead, existing work either fails to provide the visual selection query, the query conversion, the support for SEs, or the query suggestions. This is the novelty of our framework: to provide a visual analytic workspace where external VA tools provide enhanced data analysis of time-series datasets by converting visual selection queries to search queries to be used within well-known SEs and supplying query suggestions to further enhance the analysis. To promote this query conversion, we devise a novel approach using existing pattern analysis and natural language process strategies to convert user-selected findings and elements of interest to valid SQs while also providing suggestions based on the selected finding, allowing users to navigate the data and build up knowledge.


%%%%%%%% extra potential things?
% Information retrieval, on the other hand, has specialized SQ definitions which expects an input from the user in order to query within a specialized SE. But an interesting yet less researched topic is how to translate one SQ into another SQ for usage in different SEs. For instance, there is no framework which attempts to provide a visual interface for analysing the UNData dataset and by processing user-interactions, generates multiple SQs: one mathematical-based SQ to perform correlation analysis and one text-based SQ to query Wikipedia for extra information.

% Broadly speaking, VA does not restrict data mining and information retrieval and visualization into terms of SEs, but it similarly apply probing techniques to extract information from data. That said, not all techniques focus on searching for information. Areas like dimensionality reduction and data visualization provide in ways to analyse data in its macro-level or micro-level. Gapminder~\cite{rosling2012gapminderorg} is one of such tools which allows for introspection of world indicators~\cite{undata} and for discovering global misconceptions~\cite{sarma2017hans}. On the other hand, tools which focuses on searching for specific information are less prominent in the literature~\cite{??}. The vast majority uses general query platforms for information retrieval and analysis, like databases or data warehouses~\cite{zhang2012visual}, which expects queries in a standardized formats like SQL~\cite{??}. Others also use custom or domain-specific SEs~\cite{??}. Q4EDA, instead, attempts to convert one SQ format into another SQ format in order to allow tools from one side of the spectrum to communicate to others in another side. As far as we are aware, although there are attempts to automatically convert queries from one format to another~\cite{??}, all such work does this conversion with the goal to fit a single domain-specific SE~\cite{??}. Q4EDA, however, takes a different and unique approach to bridge this gap.


%%%%%%%%%%%%%%OBS
% colocar mais coisa do query suggestion
% remover EDA e usar mais IR como base aqui, deixar EDA pra use-case somente (da pra madnar coisa pra la)


==> paper/3_method.tex <==
\section{Q4EDA}
\label{sec:method}

In this paper, we present \textit{QuEry for visual Data Analysis (Q4EDA)}, a novel query conversion framework designed to enhance data exploration tasks by ingesting user's findings through visual selections and returning \textit{search queries (SQs)} which can retrieve relevant information from general-purpose \textit{search engines (SEs)}. By identifying user-driven visual selections of findings (or patterns) of interest, Q4EDA allows visualization tools to request the conversion of said selections into SQs to be used in keyword-based SEs to retrieve textual information related to the finding. Additionally, Q4EDA provides query suggestions with recommendations based on the similarity or correlation of the selected finding to other parts of the dataset under analysis. Q4EDA is specifically designed for time-series dataset collections, hence it expects the visualization tools to similarly include a time-series data as the input visual selection query.

\subsection{Overview}\label{sec:overview}

%
%Beyond that, we see a plethora of similar concepts within information retrieval when applied to different modes of communication. For instance, image search through \textit{Reverse image lookup}~\cite{reilly2017reverse} uses a similar process where images are converted to embeddings that match the expected query format of a ``image search engine''. Similarly, within data management we see the foundation of information querying through SQL~\cite{??} and databases~\cite{zhang2012visual}. All these concepts are, up to a certain extent, analogous to each other. 
%FVP: a gente precisa disso mais a frente?
%
%To simplify and better contextualize Q4EDA, we define a \textit{Search Query (SQ)} as any format of querying for information. Similarly, we define a \textit{Search Engine (SE)} as any system which can receive an SQ and retrieve information relevant or related to the query from its database(s).
%
%Given this broad definition, the stated problem Q4EDA proposes to solve still too ample. Therefore, Q4EDA focuses on exploratory data analysis of time-series datasets. Similarly, the target outputs are two keyword-based SEs: Google and Wikipedia. Further use-cases will be discussed, but by restricting our problem, we can better define Q4EDA as a framework that links data from time-series datasets, visual queries from users, and text documents from the target SEs to enable interactive retrieval of relevant information. Additionally, by focusing on well-known SEs, such as Google and Wikipedia, users will more easily be able to use Q4EDA's outputs.
%
%Yet, Q4EDA requires an external VA tool to be applied. Consider a VA tool focused in visualizing and analysing a time-series dataset. Among the many examples, Gapminder~\cite{rosling2012gapminderorg} gives a solid use-case of how users can discover findings of commonly misconceptions. However, as we discussed in Sec.~\ref{sec:related}, such solutions require error-prone extra steps from users to search for additional information over what is seen within the tool. This forces users to exit the tool and search elsewhere (e.g. Google) for such information. Q4EDA is designed to be an external dependency of such tools in order to reduce this friction with external SEs and reduce the error-prone process of depending on the user to translate their question into a SQ to be used within this external SE, or more specifically forcing users to search Google manually with their own words and potentially understanding their findings from Gapminder. 
%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%%%%%
%FVP.: esse bloco todo parece motivacao. Voce ja falou na secao anterior o que vai fazer em geral. Aqui no overview tem que explicar como. Nao precisa justificar mais a utilidade. Isso ta na introducao.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/overall.PNG}
%     \caption{Overview of Q4EDA. Q4EDA expects an external tool to input a search query from its user's visual selection (left), and the inner operations processes each data-type from the input and outputs query suggestions and formatted queries to be used on elasticsearch query engine loaded with, for instance, Wikipedia.}
%     \label{fig:overview}% ??TODO: redo! remove google and change processors
% \end{figure}

Q4EDA is structured as summarized in Fig.~\ref{fig:overview}. After a setup phase, a visualization may forward a \textit{Visual Selection Query (VQ)} to Q4EDA to be processed and converted into a \textit{Search Query (SQ)}. Q4EDA can be divided into three distinct steps: conversion, output, and suggestion. Q4EDA conversion uses the VQ's \textit{data-types}, such as numeric or categorical values. Similarly, each of Q4EDA's outputs implements the SQ specification of a target SE. Finally, Q4EDA provides query suggestions by either correlating text documents retrieved from the SE to the dataset's available data or correlating the selected time-series pattern to other available time-series within the dataset. Although what we present of Q4EDA's implementation attempts to emulate the data available within Gapminder, the framework is purposely flexible to allow for other applications, such as will be discussed.

%%%%
\begin{figure}[h]
    \centering
    \subfigure[Time-series dataset collection structure expected by Q4EDA (left) is composed of multiple time-series datasets. Each row of the many datasets are the time-series which are visualized through tools like Gapminder~\cite{gapminderusaleviz}, and a selection within such visualization (in red) comprises the \textit{Visual Selection Query (VQ)} converted by Q4EDA.] {\includegraphics[width=0.45\textwidth]{figures/vq.PNG}\label{fig:vqoverview}} 
    %%
    \subfigure[Overview of Q4EDA conversion and suggestion processes. Q4EDA expects to have access to a dataset collection and a given user's VQ (left), and the inner operations converts each data-type into output queries which are combined as a valid SQ (right). After executing the SQ in a SE and retrieving the text documents, Q4EDA also provides query suggestions.] {\includegraphics[width=0.45\textwidth]{figures/overall.PNG}\label{fig:q4edaoverview}}
    \caption{Overall summary of Q4EDA.}
    \label{fig:overview}
\end{figure}
%%%%

\subsection{Design Requirements}
\label{sec:design}

Q4EDA focuses on providing an VQ conversion framework for time-series dataset exploratory analysis. By combining elements of information retrieval, the gaps in the literature in regards to VQ conversion, and the goal stated above, we have compiled a list of requirements:

\begin{description}% add citations to most or all of them
\item[R1 -- Visual Query Conversion.] Q4EDA must provide a valid SQ given a VQ that provides: (a) \textbf{output correctness} -- the information returned from the targeted SEs should be related to the user's VQ~\cite{croft2010search}; and (b) \textbf{output stability} -- the results should not vary too much given slight variations on the VQ since slight variations of user interaction (selection) are expected to happen in practice~\cite{carpineto2012survey};
%
%
% \item[R1.a -- Output Correctness.] The information returned from the targeted SEs should be related to the user's VQ~\cite{croft2010search};
% \item[R1.b -- Output Stability.] Resulting SQ should be stable. That is, if one uses it to query SEs, the results should not vary too much given slight variations on the VQ since slight variations of user interaction can cause changes in input parameters~\cite{carpineto2012survey};
% \item[R1.c -- Framework Flexibility.] Q4EDA's design must match the expectation of a framework~\cite{??}, where it attaches to existing VA tools while adapting to multiple use-cases.

\item[R2 -- Information Retrieval.] Q4EDA should follow existing approaches to enhance the retrieved results, including: (a) \textbf{query expansion} -- the converted SQ should be expanded~\cite{azad2019query} with terms to broaden the query results to better allow for related information to be found; and (b) \textbf{query suggestion} -- suggestions~\cite{ooi2015survey} should be provided to provide users with information of interest.
%
% \item[R2.a -- Query Expansion.] Q4EDA should use query expansion~\cite{azad2019query} to populate the converted SQ;
% \item[R2.b -- Query Suggestion.] Q4EDA should provide query suggestions~\cite{ooi2015survey} by using the input and the available datasets used by the external VA tool.
\end{description}

\subsection{Q4EDA Definitions}
\label{sec:inputformal}

As a first step, it is essential to define what an SQ is in our context. Many online resources define SQ as ``A search query or search term is the actual word or string of words that a search engine user types into the search box''~\cite{keyvssq}. Beyond that, we see a plethora of similar concepts when applied to different modes of communication. To simplify and better contextualize Q4EDA, we define a \textit{Search Query (SQ)} as a term-based format of querying for information. Similarly, we define a \textit{Search Engine (SE)} as any system which can receive an SQ and retrieve information relevant or related to the query from its database(s), where among the most famous examples are Google, Wikipedia, Apache Lucene and Elasticsearch~\cite{elasticsearchwikipedia}.

% \subsection{Visual Selection}
% \label{sec:inputformal}

As we discussed, Q4EDA is designed to be used by a data analysis visualization tool to convert a \textit{visual selection query (VQ)} into a \textit{search query (SQ)}, which can then be used to retrieve information from a \textit{search engine (SE)}. For this, Q4EDA expects to have access to the \textit{time-series dataset collection} being analysed. Q4EDA also expects the data to be organized as such: the dataset collection is made up of multiple datasets wherein lives the many time-series, as is exemplified in Fig.~\ref{fig:vqoverview}. For instance, UNData~\cite{undata} is a dataset collection where multiple datasets of so called indicators (e.g. ``life expectancy'' or ``child mortality'') contains a per country time-series. With this, we have the four main \textit{data-types} of Q4EDA conversion: \textit{dataset name}, \textit{categorical descriptor} \obs{such as country name}, \textit{temporal descriptor} and \textit{time-series value}. With this, we also define a \textit{Visual Selection Query (VQ)} as a subset of a visualization's data which was selected through user interaction as exemplified as the red selection of Fig.~\ref{fig:vqoverview}. For instance, Gapminder's line-chart~\cite{gapminderusaleviz} could theoretically allow for a box-selection or lasso-selection of a part of the displayed data with which the user can indicate a visual selection query. This VQ would include the selection years as the x-axis's temporal descriptor of the selection, the y-axis's time-series numeric values and the corresponding dataset name and categorical descriptor of that individual line-chart.

With these definitions in hand, we can describe Q4EDA as a framework that receives a VQ and, by utilizing the available dataset, it converts the VQ into one of the output SQ formats. After executing said SQ, Q4EDA also provides query suggestions among the available dataset names and categorical descriptors. For that, the workflow to use Q4EDA follows the representation of Fig.~\ref{fig:overview} where after a user performs a VQ, its data is given to Q4EDA for the query conversion and suggestion process.

% Throughout this work, we will constantly reference Gapminder and its underlying datasets. 
% %
% %FVP.: precisa mesmo usar o gapminder aqui? Nao pode ser generico e depois especilizar? Country seria parte dos metadados. Lembro de termos conversado isso. Na frente, quando metadados tinha algo relacioando a paises, discutiamos como converter.
% %
% We define the whole UNData~\cite{undata} dataset of world demographic indicators is defined as $I$, where $I$ can be partitioned through $C$ countries and $D$ unique indicators. Each combination of country and indicator $I^d_c$ is composed by a set of time-series defined as ${I^d_c=\{e_{t_1}, \ldots, e_{t_n}\}}$, where $e$ is each data-point entry measured among $\{y_1, \ldots, y_n\}$ years. In this context, the visual selection query is expected to refer to one or more indicators $d$, one or more countries $c$, and one or more years $y$. This selection will be referenced as \textit{finding} $F$ for the remainder of the paper and is defined as $F \subset I$. 
% %
% For instance, if a line-chart visualization is used~\cite{gapminderusaleviz}, the selection would be $F=I^d_c(y_a, y_b)=\{e_{y_a}, \ldots, e_{y_b}\}$ where a range of years $y_1<=y_a<y_b<=y_n$ is selected from a single combination of indicator $d$ and country $c$. Fig.~\ref{??} shows an example of selecting a finding, which is displayed as a gray area -- a massive decrease in the ``Life Expectancy'' of ``United States'' in the period between $1917$ and $1919$. Of course, different visual metaphors would change the variables that are a range and not. For example, if we consider Gapminder's bubble-chart, the expected selection would have a range of countries, two indicators, and a single year. While Q4EDA does not attempt to limit what visual metaphor is being used by the external VA tool, it does expect the input of which variables were part of the visual selection itself $V$ versus which were not.
%
%FVP.: aqui tentaria ser generico, colocando exemplos, que podem ser do Gapminder, para exemplificar.
%

\subsection{Query Conversion}
\label{sec:queryspec}

Q4EDA's framework leans on the three aspects: \textit{query conversion}, \textit{query combiner}, and \textit{query suggestion}, as is seen in Fig.~\ref{fig:overview}. While the query combiner defines the supported SEs, the query conversions defines the process used to convert each of VQ's individual data-types to generate a relevant output SQ using query expansion techniques (\textit{R2.a}). For this, Q4EDA first converts each data-type separately, and then the results are \textit{combined} and \textit{formatted} into the output SQ.

The inner mechanism used by Q4EDA to process and store the individual conversion step follows a grammatical convention based on existing SQ grammars, the closest of which is the Elasticsearch's Simple Query format~\cite{SimpleElastic}. The formal grammar described in EBNF~\cite{feynman2016ebnf} is:

\setlength{\grammarparsep}{1pt plus 1pt minus 1pt} % change separation between rules
\begin{grammar}\label{grammar}
<sub-expression> ::= <or> | <and> | <required> | <term>

<or> ::= `(' <sub-expression> \{ `|' <sub-expression> \}+ ')'

<and> ::= `(' <sub-expression> \{ `&' <sub-expression> \}+ ')'

<required> ::= `\"'  <sub-expression> `\"'

<term> ::= [<negative-factor>] <inner-term> [<weight-factor>]

<inner-term> ::= `(' <spaced-term> `)' | <word>

<spaced-term> ::= <spaced-term> ` ' <word> | <word>

<word> ::= \{ <lower-case-letter> \}+

<weight-factor> ::= superscript ? <weight-factor>

<negative-factor> ::= `-'
\end{grammar}

where the conversion's \textit{sub-expression} output consists of multiple \textit{terms} which can represent the input \textit{positively} or \textit{negatively}, and with the added \textit{weights} and logical operations, the output is able to be descriptive enough for formatting to target many SEs. In order to exemplify the grammar, if we consider an input which is requesting Q4EDA to convert the question ``population of the United States'' into a SQ, a plausible output could be $\{ (\text{united states} \mid \text{usa} \mid \text{america} \mid (\text{north america})^{0.5}) \& (\text{population} \mid \text{habitants} \mid \text{people}^{0.5} \mid (-\text{death})^{0.5} ) \}$, where it includes perfect match terms (e.g. ``united states''), terms with lower weights for less exact matches (e.g. ``north america'') and negative terms to indicate opposite meaning or antonyms (e.g. ``death'').


\subsubsection{Keyword Conversion}
\label{sec:indicatortags}

The first conversion tackles the keyword data-type, such as the dataset name or categorical descriptors. By acquiring the dataset name(s) from a given VQ or the categorical descriptor(s), Q4EDA uses natural language processing to generate a set of related terms for inclusion in its output. We first apply a text mining approach to assign a set of related terms $T^D_d=\{t_1^d, t_2^d, \ldots\}$ for every keyword $d$ received. For instance, the keyword $d=\text{``life expectancy''}$, which is a dataset name from UNData~\cite{undata}, besides of being represented by the terms ``life'' and ``expectancy'', can also be represented by terms like ``longevity'' and ``lifetime''. Similarly, the same keyword is negatively represented by terms like ``mortality'' or ``death''. Such an example results in the terms $T^D_{life\_expectancy}=\{life, expectancy, longevity, lifetime, -mortality, -death\}$ where positive terms are related to the keyword, and negative terms are negatively related, a concept similar to antonyms. In this way, any such nominal descriptors will have its semantic meaning defined by its associated terms. Finally, the set of terms are formatted into an expression following Q4EDA's grammar: $(life \| expectancy \| longevity \| lifetime \| -mortality \| -death)$.

This operation is done through a pre-trained GloVe model~\cite{pennington2014glove} which generates related tags for a given keyword. First, the GloVe model is loaded using the Gensim library~\cite{rehurek2011gensim}, and then every unique keyword $d$ is tokenized and lemmatized with NLTK~\cite{loper2002nltk} and WordNet~\cite{fellbaum2010wordnet, zhang2009concept} and passed to Gensim's ``similar\_by\_vector'' method.

\subsubsection{Country Keyword Conversion}
\label{sec:geolocal}

Although the simple method described so far works well for dataset names and categorical descriptors with common nouns, specialized versions of keyword conversion are used to dataset names or categorical descriptors with proper nouns, such as geo-locations such as street, building name, city, state or country and events such as ``the second world war'', for better query expansion results~\cite{bhogal2007review}. Therefore, Q4EDA provides one of such specialized keyword conversions to properly process a country keyword.

Since geo-information also encodes geographical concepts like continents, distances, area, population, among others, this specialized conversion can output a more relevant set of terms for a given country. That said, this module design could expand indefinitely due to its data complexity, therefore we limited our processing to grammatical variations, naming conventions, synonyms, and regionality. To create the set of terms $T^C_c$ of words for a country keyword, the country's name is used along with other terms related to the country, such as adjectives or nouns (e.g. ``United States'' adds ``America'', ``American'' and ``USA''). Although a VQ may be specific for a single country, the VQ's relevant information within the target SE may include other similar or neighboring countries as well. Therefore, we add terms for the collection of countries nearby the selected country, such as the continent name or sub-area, with a smaller weight (e.g. ``United States'' adds ``North America'' with lower weights). This generalization has shown to be essential because some textual information may only contain more general references to the geographical location where a specific event occurred. To complement $T^C_c$ with said extra data, we extracted data from Gapminder's geography dataset~\cite{gapmindergeography} and used it as a reference for any country \textit{categorical descriptor}, such as is the case with UNData. Therefore, such an example results in the following output:
\begin{align*}
T^C_{united\_states} = &(\text{united states} \mid \text{united states of america} \mid \\
& \text{american} \mid \text{america} \mid \text{usa} \mid (\text{north america})^{0.5})
\end{align*}
Finally, the list of terms is converted to Q4EDA inner grammar definition.

\subsubsection{Temporal Descriptor Conversion}
\label{sec:temporal}

Unlike previous processors, the temporal descriptor conversion is unique since it tackles a continuous temporal value and has some inner context that can be used to enhance search queries. Similar to the country keyword conversion, this step is required to be specialized to a given temporal variable, such as date, time, month, week-day, year or any combination of them. Therefore, Q4EDA provides one of such implementations which focuses on converting a year range into a valid query output to be included in Q4EDA's output SQ.

The term set generated has the form of $T^E_{y_a, y_b}=\{t_1^e, t_2^e, \ldots\}$ where $y_a$ and $y_b$ identify the limits of the range of years. The natural terms associated with a range of years are the years themselves. However, this conversion process goes beyond and allows the VA Tool to define a weight distribution to better describe the selection interest within the range of years. For instance, while the default weight profile will give the same weight to all years within a range, if the VA Tool includes a gaussian weight distribution, the processor will give higher weights to the center of the range and lower to the others.

Additionally, the year conversion compares the year range to a predefined year range term. For example, if the year range is $1950--1960$, an additional term of $1950s$ is included to represent the decade selected. If the year range does not match the exact decade, lower weights are given to the decade terms. The weight used in decade terms is $w=1-2*(|ds^b_a| + |ds^e_b|)$ where $ds^b_a$ is the distance from the first year to the beginning of the decade and $ds^e_b$ is the distance in years from the last year to the end of the decade, and weights equal or below $0$ causes the decade term to be discarded. The same process is applied for centuries. Therefore, such an example results in the following output:
\begin{align*}
T^E_{1851--1859, gaussian} =& (1851^{0.2} \mid 1852^{0.3} \mid 1853^{0.5} \mid 1854^{0.8} \mid 1855 \mid  \\
& 1856^{0.8} \mid 1857^{0.5} \mid 1858^{0.3} \mid 1859^{0.2} \mid 1850s^{0.6})
\end{align*}

\subsubsection{Time-Series' Selected Finding Conversion}
\label{sec:patterndetection}

Finally, we analyse the numerical values selected by the user $F=I^d_c(y_a, y_b)=\{e_{y_a}, \ldots, e_{y_b}\}$ and converts the underlying pattern into a set of terms $\{t_1^p, t_2^p, \ldots\}$. Our implementation categorizes the selected values, which we call \textit{finding}, by its trend $tr$, which can be either \textit{ascending}, \textit{descending} or \textit{stable}, and by its pattern $tp$, which can either be \textit{peak}, \textit{valley}, and \textit{neutral}. This results in $9$ different possible trend/pattern combinations, as exemplified by Fig.~\ref{fig:detectionpossibilities}. These two identifiers are applied to a finding by using existing trend/pattern statistical methods and the resulting keyword is then converted to the desired query output using the same GloVe model~\cite{pennington2014glove} NLP process used in the Keyword Conversion (see Sec.~\ref{sec:indicatortags}). That said, if the input has only one value (e.g. $a == b$) or no value, this conversion step will output nothing at all.

%%%%
\begin{figure}[h]
    \centering
    \subfigure[Combinations of trends and patterns types in visual selections.] {\includegraphics[width=4.25cm]{figures/detectionpossibilities2.png}\label{fig:detectionpossibilities}}\quad
    %%
    \subfigure[Peaks and valleys detection.] {\includegraphics[width=4.25cm, height=3.4cm]{figures/peakdetectionexample.PNG}\label{fig:patternpossibilities}} 
    \caption{Examples of trends and patterns combinations and peaks and valleys detected by our algorithm.}
    \label{fig:patternpossibilitiesoverview}
\end{figure}
%%%%

The type of a selected trend $tr$ is defined by applying the Moving Averages (MA) method, a well-known technique in time-series analysis to define whether a series is stationary or not, providing us with a trend estimation~\cite{brockwell2016introduction}. MA first transforms the selection $F=I^d_c(y_a, y_b)=\{e_{y_a}, \ldots, e_{y_b}\}$ into a new series $F'=I'^d_c(y_a, y_b)=\{e'_{y_a}, \ldots, e'_{y_b}\}$ setting its values $e' \in I'^d_c(y_a, y_b)$ to the average value in the time interval $e'_p(w) = \mu( e_{y-w}, \ldots, e_y, \ldots, e_{y+w})$. Here we empirically define the window with the default value $w=2$, however it is possible to modify this parameter during setup. After that, we compute the discrete derivative of $F'$ and sum the normalized values as follows

\begin{equation}
    \label{eq:diffMA}
    tr = \sum_{{e'}_y \in {F'}} \frac{{e'}_y - {e'}_{y-1}}{|{e'}_y - {e'}_{y-1}|}.
\end{equation}

Based on that, the trend type is defined as

\begin{equation}
    \label{eq:pattern1}
    trend = \left\{
    \begin{array}{ll}
        \text{ascending},  & tr > 0           \\
        \text{descending}, & tr < 0           \\
        \text{neutral},    & \text{otherwise} \\
    \end{array}
    \right.\text{.}
\end{equation}

To define the pattern type $tp$ of the selected finding, we use peak detection methods which attempt to identify a local maximum by comparing neighboring values~\cite{virtanen2020scipy, Yang2009ComparisonAnalysis}. In this process, we identify all $k_p$ potential peaks within the selection, and similarly, we identify all $k_v$ potential valleys by inverting the selection data points as $F_v=-F=-I^d_c(y_a, y_b)$. Using this method, we assign a pattern factor $pf$ to the selection $F$, computing the following equation to determine whether it contains a peak, a valley, or neither.

\begin{equation}
    \label{eq:peaksfw}
    \begin{array}{ll}
        pf = |F| \times \frac{(w^+ - w^-)}{\sigma(F)}\text{, } \\
        w^+ = \sum_{k_p}W(k_p).Pr(k_p), k_p \in peaks\text{, } \\ 
        w^- = \sum_{k_v}W(k_n).Pr(k_v), k_v \in valleys\text{, } \\ 
    \end{array}
\end{equation}

In equation Eq.~(\ref{eq:peaksfw}), $W$ represents the width and $Pr$ the prominence, or absolute height, of the peak or valley. Therefore $w^+$ is equivalent to a probability of the selection to be a peak and $w^-$ a similar probability of being a valley. Note that $\sigma(F)$ is the standard deviation of $F=I^d_c(y_a, y_b)$. Based on the pattern factor $pf$, the type of pattern is defined as

\begin{equation}
    \label{eq:seconddegree}
    pattern = \left\{
    \begin{array}{ll}
        \text{stable}, & \sigma(F^r_c) < \lambda_1\\
        %\text{---}, & \sigma(F^r_c) < \lambda_1\\
        \text{peak},     & \sigma(F) > \lambda_1 \text{ and } pf > \lambda_2                    \\
        \text{valley},   & \sigma(F) > \lambda_1 \text{ and } pf < -\lambda_2                   \\
        \text{unstable}, & \sigma(F) > \lambda_1 \text{ and } \lambda_2 \geq pf \geq -\lambda_2
    \end{array}
    \right.\text{, }
\end{equation}
where $\lambda_1$ is a threshold of whether to consider if a selection contains a pattern or not, and, if a pattern is detected, $\lambda_2$ is a threshold to define whether the selection is a peak, a valley, or an unstable oscillation. Empirically we set $\lambda_1 = 0.5$ and $\lambda_2 = 1.5$, but these parameters can be changed.

The result of this process is a pair of identifiers ($trend$ and $pattern$), which describes the selection and is exemplified in Fig.~\ref{fig:patternpossibilities}. Finally, we define the conversion's output by using the identifier pair as keywords to be converted with the same GloVe model presented in Sec.~\ref{sec:indicatortags}, in which Q4EDA expands a keyword into a valid query output to be used within the output SQ.
%Also similar to NoP, the VA Tool has access to these terms and is able to change them if required. For example, this process generated the terms $\{high, peak, boom, boost\}$ from a \textit{stable} and \textit{peak} finding, and $\{increase, higher, growth\}$ from a \textit{ascending} and \textit{neutral} finding. % TODO: REMOVE??
% Finally, the list of terms is converted to Q4EDA inner grammar definition similar to previous processors.

\subsection{Query Combiner and Output Formatter}

So far, we exemplified the conversion process given a singular input to each. Each conversion outputs a single query output in the sub-expression format of Sec.~\ref{sec:queryspec}, with a valid sub-expression representing that specific. However, Q4EDA is not limited to only one input per data-type. Instead, each conversion process is done for \textbf{each occurrence of its input}, therefore if the input has multiple datasets $\{D1, D2, \eta\}$, the keyword conversion will be executed for each individual dataset name and return one sub-expression per dataset $T^{D1}, T^{D2}, \eta$. All other processors would similarly be executed multiple times if the VQ includes multiple occurrences of the input metadata types. 

Q4EDA then combines every sub-expression into a full expression by first creating a full combinatory permutation within each sub-expression output excluding the time-series pattern conversion, since its output will already be associated to the combination the others. For instance, if the VQ contains two countries, one dataset name and two ranges of years, then Q4EDA would also expect four finding sub-expressions, one for each of the country/name/years combination. With this, each of the two countries would be converted individually $T^C_{c1}$ and $T^C_{c2}$, the dataset name would be converted to $T^D_{d}$, the two year ranges of the selection would output $T^E_{y_a, y_b}$ and $T^E_{y_c, y_d}$, and the four findings would output four distinct $T^P$. Q4EDA then expands the combinatory permutations as four inner queries by the combinatory permutations one by one and concatenates each with an ``and'' $\&$ operation, resulting in the following four sets of sub-expressions: $(T^C_{c1} \& T^D_d \& T^E_{y_a, y_b} \& T^P_{c1, d, y_a, y_b})$,  $(T^C_{c1} \& T^D_d \& T^E_{y_c, y_d} \& T^P_{c1, d, y_c, y_d})$,  $(T^C_{c2} \& T^D_d \& T^E_{y_a, y_b} \& T^P_{c2, d, y_a, y_b})$ and $(T^C_{c2} \& T^D_d \& T^E_{y_c, y_d} \& T^P_{c2, d, y_d, y_c})$. 

Then, to unite the sub-expression sets, two expressions are calculated: a full expression intersection $T_I$ by concatenating all sub-expressions sets with ``and'' $\&$ operands and a full expression union $T_U$ by concatenating all sub-expression sets with ``or'' $\|$ operands. These two are then united as $T = (T_I)^2 \| T_U$ where the full intersection is given higher weight over the full union. Note that $(T_I)^2$ applies a weight operation to an sub-expression set instead of an inner-term, as defined by our grammar. Therefore, every term within the full expression intersection should have its weight multiplied by $2$. Finally, the two full expressions are summarized through a Boolean Algebra~\cite{lashkari2009boolean} which includes Exponentiation Algebra to also solve for the weight-factor calculation.
% do I explain more? I'm not sure if it is needed..

Finally, we use an output formatter to reformat the final query calculated above into a valid SQ of a given SE. Q4EDA provides one such formatter which converts the query to the Elasticsearch simple query format~\cite{SimpleElastic} by replacing the following aspects of the query:

\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{lll}
\toprule
\textbf{bnf} & \textbf{inner example} & \textbf{elasticsearch equivalent} \\ \hline
weight-factor & superscript & $\wedge$  \\
negative-factor & $-$ & N/A \\
and & $\&$ & $+$ \\
required & ``spaced term'' & +(spaced term) \\
spaced-term & some words & ``some words'' \\
%   &  & \\ \hline
\bottomrule
\end{tabular}
\end{table}

therefore, other than the direct equivalents listed above, which are simply replaced, the \textit{negative-factor} is not available and removed. Note that the term itself with a \textit{negative-factor} is kept as regular \textit{operands} (e.g. ``$(-mexico^{0.5})$'' becomes ``$mexico^{0.5}$'') since querying for antonym terms of the finding can also represent information about it~\cite{zhang2009concept}.

% %%%%%%%%
% %%%%%%%%
% %%%%%%%%
% %FVP: acho que deveriamos focar no elastic search e comentar mais no final a adaptacao para o google em discussoes. Vai ficar muito confuso colocar tudo isso aqui.


% \textbf{Google. } By following the google search grammar~\cite{googlesearch}, the google output module simplifies the final inner query to the components also supported by google search. Namely, the changes are: %LC: TODO: move this to discussion very small and remove google from method

% \begin{table}[ht]
% \centering
% \begin{tabular}{lll}
% \toprule
% bnf & inner grammar & google equivalent \\ \hline
% weight-factor & superscript & order of terms \\
% negative-factor & $-$ & N/A \\
% and & $\&$ & AND \\
% or & $|$ & OR \\
%   &  & \\ \hline
% \end{tabular}
% \end{table}

% therefore, higher weighted terms are moved towards the beginning of the search query, the listed operands are replaced by their google equivalents and all \textit{negative-factor} and \textit{weight-factor} occurrences are removed. Note that the \textit{operands} with \textit{negative-factor} or \textit{weight-factor} are not removed, but kept as regular \textit{operands} (e.g. ``$(-mexico^0.5)$'' becomes ``$mexico$'') since querying for antonym terms of the finding can also represent information about it~\cite{zhang2009concept}.

% \textbf{Elasticsearch. } The Wikipedia output is similarly done by following elasticsearch's simple query format~\cite{SimpleElastic}. Namely, the changes are:

% \begin{table}[ht]
% \centering
% \begin{tabular}{lll}
% \toprule
% bnf & inner example & elasticsearch equivalent \\ \hline
% weight-factor & superscript & \wedge  \\
% negative-factor & $-$ & N/A \\
% and & $\&$ & $+$ \\
% required & ``spaced term'' & +(spaced term) \\
% spaced-term & some words & ``some words'' \\
%   &  & \\ \hline
% \end{tabular}
% \end{table}

% therefore, other than the direct equivalents, which are simply replaced, the \textit{negative-factor} is once again not available and removed as was with the google output module.
% %%%%%%%%
% %%%%%%%%
% %%%%%%%%


%%%%%%%%%%%%%%%

\subsection{Query Suggestion}\label{sec:correlation}

In parallel to the SQ conversion, Q4EDA also provides query suggestions by utilizing and analyzing the available dataset collection, the VQ and the final text documents results from the conversion process, as is shown in Fig.~\ref{fig:overview}. In other words, Q4EDA not only implements query expansion (\textit{R2.a}) by aggregating relevant terms to the SQ through the conversion processes but also implements query suggestions (\textit{R2.b}) in terms of the visual selection query by suggesting other partitions of the dataset collection which may potentially be related. By loosely following information retrieval techniques~\cite{ooi2015survey}, Q4EDA tackles two suggestion approaches where users are suggested related dataset names and categorical descriptors. First it provides suggestion given the presence of said dataset names or categorical descriptors within the text documents which were retrieved from the SE after executing the final SQ. Second, Q4EDA provides suggestions based on the numerical or pattern similarity of the VQ finding to other possible VQs among all the datasets and categorical descriptors.

\subsubsection{Nominal Suggestions from Text}
\label{sec:NST}

The first suggestion approach attempts to search the available nominal data's presence, which includes both the dataset name and the categorical descriptor, in a given text document. For that, a VQ is required to be converted and its output SQ executed within the target SE. The resulting text document(s) are used by this suggestion process to rank the nominal data present on each text document by number of occurrences. The result provides the suggestion of other datasets or categorical descriptors which are related to the text document being read. In order to broaden the use of this suggestion approach, we provide three implementations: direct counting, indirect counting and natural language processing (NLP), and the result is a score list which associates each nominal data to each of the texts. That is, if we follow the previous sections' examples, Q4EDA suggests the most relevant datasets and countries within UNData that relates to any given Wikipedia text document which was retrieved from Elasticsearch after executing the result of a VQ conversion.

In the direct mode, we use a simple case-insensitive number of occurrences of all possible nominal data from the dataset, or, in other words, we apply a bag-of-words technique. That is, Q4EDA suggests a ranked list indicating the number of occurrences of every dataset name and another ranked list for the categorical descriptor. In the indirect mode, however, we first use the same keyword conversion approach of Sec.~\ref{sec:indicatortags} to expand the available keywords from the dataset name and categorical descriptor, and their query output's terms are then searched within the text document using bag-of-words. 
%After searching each s terms within the document, Q4EDA also uses the negative-factors and weight-factors of said sub-expression to calculate the final \textit{suggestion score} between the nominal metadata and the text document. 
Finally, with the nlp mode, we compare the keyword conversion outputs to an the extracted keyword list from the text document through another NLP method called which Gensim Keywords~\cite{rehurek2011gensim} which transforms text documents into keywords. Finally, we once again use NLTK with the GloVe model~\cite{pennington2014glove} to transform both sets of terms, namely the keyword conversion and from the text keyword extraction, into two vector embeddings which are then compared with cosine \obs{similarity}. The result is, once again, one ranked list per nominal data which indicates suggestions indicating the similarity between the text contents and the available data within the dataset collection under analysis.

To exemplify our approach, if we assume Q4EDA setup with Elasticsearch's Wikipedia Dump~\cite{cirrussearch}, UNData~\cite{undata} and Gapminder line-charts~\cite{gapminderusaleviz}, and at some point the user performs a VQ which, after converted and executed, returns a Wikipedia document about USA's life expectancy, then we scan the whole UNData dataset collection across the two nominal data, namely dataset name and country, and search for all their keywords (e.g., United States or Life Expectancy) within the text document. In the direct mode, we would provide two lists containing number of occurrences of each country and indicator within the text documents. In indirect mode, we convert each dataset name and country using the keyword conversion process and search the resulting terms (e.g., United States, USA, American for the united states country or Life, Expectancy, Death for the life expectancy indicator) within the text document, and the occurrences of each term is aggregated as its respective dataset name or country as an average. The results are similarly two lists indicating the average occurrences of related terms of each country and dataset name. Finally, with the NLP mode we also convert the text document itself into a keyword list and by converting both this list and the keyword conversion query output terms to a vector embedding format, we calculate their cosine similarity. Once again, the results are two lists indicating a similarity score between the text's generated keywords and the related terms of each country and dataset name. Independent of the mode used, the resulting lists are a country ranking list of the most related countries to the text and an indicator list of the most related indicators to the text documents.

While the direct mode provides suggestions of other nominal data present in the text and the indirect mode provides suggestions of other nominal data whose concept is present in the text, the NLP mode provides suggestions of nominal metadata whose concept matches the most prominent concepts within the text. In other words, the direct mode is better to find texts literally talking about ``life expectancy'', the indirect mode is better to find texts with information that talks about the concepts surrounding ``life expectancy'' of a country (e.g. including ``death'' and ``mortality''), and the NLP mode is better to find texts whose overall context is regarding the concepts surrounding ``life expectancy'' of a country. In the case of suggesting UNData nominal data from Wikipedia text documents, through our preliminary tests we gathered that the direct mode provided better ways to suggest nominal data based on the presence of specific words within the text, such as ``child'' of the child mortality indicator, the indirect mode provided better ways to suggest similar countries of a given VQ, and the NLP mode provided better ways to suggest similar datasets of a given VQ.


%Similarly, with datasets such as the NYC-taxi-trip~\cite{nycdataset} or DJIA 30 Stock~\cite{stockdataset}, Q4EDA can find occurrences of nominal metadata (e.g., driver id or stock code) within textual inputs (e.g., google short descriptions or tweets from Twitter) and suggest the nominal metadata related to the text.

% For instance, if Q4EDA is setup with the UNData~\cite{undata} and, at some point, it receives a text document about USA's life expectancy as a text document input, then NSTd scans the whole UNData dataset across the two nominal metadata (e.g., country and indicator), and search all their keywords (e.g., United States or Life Expectancy) within the text document, returning the number of matches for each possible country and indicator. Similarly, with datasets such as the NYC-taxi-trip~\cite{nycdataset} or DJIA 30 Stock~\cite{stockdataset}, Q4EDA can find occurrences of nominal metadata (e.g., driver id or stock code) within textual inputs (e.g., google short descriptions or tweets from Twitter) and suggest the nominal metadata related to the text.

% Assuming an external VA tool is attached to Q4EDA, it is able to first convert visual selection query to a SQ, use Elasticsearch to retrieve documents related to the visual selection query, then use these text documents as inputs to NSTd to provide suggestions to their user of which other nominal metadata are present within the documents. Furthermore, if such example is the Gapminder VA tool~\cite{gapminderusaleviz} and an Elasticsearch setup with Wikipedia documents~\cite{cirrussearch}, then NSTd provides suggestions of other related countries or indicators to the visual selection for further exploration pathways.

% \subsubsection{Nominal Suggestions from Text indirectly (NSTi)}
% \label{sec:NSTi}

% A suggestion module similar to \textit{NSTd} is \textit{NSTi}, where instead of searching directly for the nominal terms within the text document, it uses NLP techniques as an interface between the two. 
% %
% %FVP que texto e que two data-types? LC: tirei data-types.. two eh nominal terms e text documents (logo antes na frase)
% %
% The goal with \textit{NSTi} is the same as \textit{NSTd}. However, in addition to gathering all nominal metadata from the dataset, NSTi uses the respective nominal processor's sub-expression output as the terms to search within the text document. After searching each sub-expression's terms within the document, Q4EDA also uses the negative-factors and weight-factors of said sub-expression to calculate the final \textit{suggestion score} between the nominal metadata and the text document. 

% For instance, if Q4EDA is once again setup with the UNData~\cite{undata} and, at some point, it receives a text document about USA's life expectancy as a text document input, then NSTi scans the whole UNData dataset across the two nominal metadata (e.g., country and indicator) and also converts each nominal metadata using the corresponding NoP to expand the terms of that nominal metadata. Finally, NSTi searches the text document for each individual term of the sub-expressions (e.g., United States, USA, American for the united states country or Life, Expectancy, Death for the life expectancy indicator) within the text document. For each sub-expression, the number of matches of each term is applied to its respective weight and negative factors and the average of such values is computed into a final score. The result will be a list of the relationship scores of each individual nominal metadata to the text document, which when considering the UNData could be a country ranking list of the most related countries to the text and an indicator list of the most related indicators to the text. If we assume the same setup with Wikipedia documents~\cite{cirrussearch}, such lists are suggestions provided by NSTi of countries and indicators related to the visual selection.

% % Through our preliminary tests, \textit{NSTi} seemed more useful in scenarios where the user wished to find ``similar documents'' to a certain selection, while \textit{NSTd} seemed more useful when users wished to find ``documents talking about the specific occurrence''. For example, \textit{NSTd} is better to find texts literally talking about ``life expectancy'' while \textit{NSTi} is better to find texts with information that talks about the concepts surrounding ``life expectancy'' of a country (e.g. including ``death'', ``mortality'', ...).


% \subsubsection{Nominal Suggestions from Text through NLTP (NSTnltp)}

% Following the previous two suggestion modules, Q4EDA provides a third suggestion module that uses the same process of \textit{NSTi} to process the nominal metadata. However, instead of using bag-of-words, \textit{NSTnltp} applies \textit{NLP} to the text input as well. For this, first, Q4EDA expects a text document input and by extracting the dataset's nominal metadata and executing their respective processors as is done by NSTi, NSTnltp compares the sub-expression terms to the extracted text document's keywords extracted through an NLP method. NSTnltp provides one main NLP method to transform the text documents into a list of keywords: Gensim Keywords~\cite{rehurek2011gensim}. Since Gensim Keywords does not need any training step with a specific text dataset, it is does not limit the model's applicability to text documents only from the domain of the training dataset, and its execution is fast in order to process many text documents at once. Finally, NSTnltp use this keywords list as the means of comparison between the nominal metadata sub-expressions and the text document. We once again use NLTK with the GloVe model~\cite{pennington2014glove} to convert the sub-expression terms and the text keywords into two embedded vectors and apply cosine dissimilarity to compare the two vectors. The NSTi provides the resulting similarity value lists per each nominal metadata as query suggestions.

% Following the examples of previous modules, if Q4EDA is once again setup with the UNData~\cite{undata} and, at some point, it receives a text document about USA's life expectancy as a text document input, then other than all the process done by NSTi, NSTnltp also converts the text into a keyword list and converted to a vector embedding. For each sub-expression, the terms are also converted into vector embeddings and compared to the keyword list vector though cosine dissimilarity. Similar to before, the result will be a list of the relationship scores of each individual nominal metadata to the text document, which when considering the UNData could be a country ranking list of the most related countries to the text and an indicator list of the most related indicators to the text. With this, \textit{NSTnltp} calculates a list of the similarity score of nominal values that are ``semantically'' related to the text and its result can once again be used by the VA Tool for visualization or suggestion purposes. 

% Though this module's purpose is similar to the previous two, the output's suggestion of each provides different query suggestions. While NSTd provides suggestions of other nominal metadata literally present in the text and NSTi provides suggestions of other nominal metadata whose concept is present in the text, NSTnltp provides suggestions of nominal metadata whose concept matches the concepts within the text. In other words. \textit{NSTd} is better to find texts literally talking about ``life expectancy'', \textit{NSTi} is better to find texts with information that talks about the concepts surrounding ``life expectancy'' of a country (e.g. including ``death'', ``mortality'', ...), and \textit{NSTnltp} is better to find texts whose overall context is regarding the concepts surrounding ``life expectancy'' of a country. In the case of suggesting UNData nominal metadata from Wikipedia text documents, through our preliminary tests we gathered that NSTd provided better ways to suggest nominal metadata based on the presence of specific words within the text, such as ``child'' of the child mortality indicator, NSTi provided better ways to suggest similar countries given a visual selection query and NSTnltp provided better ways to suggest similar indicators given a visual selection query.


% , which is quick to process but less accurate, LDA, which is also quick but is specialized to Wikipedia documents, or DistilBert, which is much slower to process but more accurate in its results.

% Although use-cases of time-series analysis normally involve well-structured data, such as tabular data, sometimes textual data is also included. Therefore, Q4EDA also has a Natural Language Text Processor (NLTP), which, similar to other processors, extracts relevant terms from a given text. The NLTP Processor has tree modes: Gensim Keywords~\cite{rehurek2011gensim}, Latent Dirichlet Allocation (LDA)~\cite{blei2003latent}, and DistilBert~\cite{reimers-2019-sentence-bert}.
% %
% %FVP.: para que tem tres modes? qual a necessidade?
% %
% %FVP.: isso daqui nao é para transformar os metadados textuais em keywords??? Fiquei meio perdido. Acho que temos que deixar claro a distinçao entre dados e metadados
% %



% For the LDA mode, given an VQ with textual input, the processor uses a loose interpretation of the work by \citet{dahir2021query}, where topics are extracted from the text using a Latent Dirichlet Allocation (LDA)~\cite{blei2003latent} model. We initially trained the model using the entire Wikipedia corpus while removing terms that occur in less than $15$ documents and terms that occur in more than $50\%$ of the documents. We empirically set these values following the common practice. This set of terms is used as the output for the NLTP, and the scores of each term are included as the weight factor for each individual term. 
% %
% %FVP: aqui fica especifico para wikipedia. E se a gente estiver usando Google. O processo é o mesmo? Precisa pensar em como generalisar. Contudo, ainda precisamos de LDA?
% %

% Finally, the DistilBert mode is somewhat more involved. Though our approach is different from related works~\cite{alhamzeh2021distilbert}, the concept of using DistilBert for query expansion follows a similar pattern. NLTP passes each document over a DistilBert pre-trained model~\cite{reimers-2019-sentence-bert} and the result is compared to TfidfVectorizer~\cite{manning2008introduction, baeza1999modern} through a cosine similarity distance. Our method is a custom re-implementation of KeyBert's implementation of contextual keyphrase retrieval with self-labeling~\cite{sharma2019self, keybertgithub} with an added GPU optimization for better response-time, providing a better user experience. The resulting term list is then used as the output for the processor.

% %FVP: nao sei se precisa falar disso aqui. a gente mostra?
% %
% %Although the results of these processors will be used to compute the final SQ, these terms have been shown to have additional applications. For instance, the VA tool can use these terms as a keyword/document matrix visualization or as a WordCloud. If multiple texts are inputted, the external tool can also create overview or text comparison visualizations, where the presence of terms among multiple text documents are encoded as visual metaphors to summarize the contents of each text. Further use of this processor will be described among the implemented query suggestion modules.

% %FPV.: essa secao ficou meio estranha porque nao da para entender o que estamos gerando. Qual part da query isso se refere.

% %FVP.: na verdade, nao fica claro como a gente ta gerando a query com esses processors


%
%FVP.: o problema de dar muitas opcoes e nao saber o que de fato é usado. Minha sugestao é definir uma e usa-la
%


\subsubsection{Nominal Suggestions from Pattern} % LC: TODO: acrecentar a ideia que vamos limitar pra 2 niveis e acrecentar a figura do cubo!
\label{sec:CSP}

The other query suggestion approach focuses on analyzing the selected finding of Sec.~\ref{sec:patterndetection} and providing related nominal data, such as dataset name or categorical descriptor, as suggestions for further analysis due to their similarity or dissimilarity. By comparing the time-series numeric values of the finding $F=I^d_c(y_a, y_b)=\{e_{y_a}, \ldots, e_{y_b}\}$ to all other equivalent findings among the nominal data present within the dataset collection, we are able to calculate a similarity list for each nominal data using statistical correlation techniques, as is exemplified in Fig.~\ref{fig:findingsuggestions}. For instance, if considering the UNData, we would output one list indicating the similarity of the finding of all other countries $c' \in C, c' \notin c$ if all other inputs are the same, which includes the year range and dataset name, and another similarity list of all other datasets $d' \in D, d' \notin d$ if all other inputs remain the same, this time including the year range and country. Among the two lists, the most similar are suggested as related to the VQ, while the most dissimilar (e.g. lowest similarity score) are suggested as examples of an ``opposite'' or ``inverted'' pattern to the VQ.

For this, we provide two different strategies to compute the aforementioned similarity: Pearson correlation and Dynamic Time-Warping (DTW)~\cite{keogh2005exact, muller2007dynamic}. These two techniques are provided because each one solves the limitations of the other. For instance, Pearson Correlation is the choice if one prefers to compare findings purely according to their general visual pattern similarity while not focusing on the distance between the selection's individual values. However, if one wishes to compare findings according to differences in amplitude or consider their raw value distances, DTW is the option. The Pearson correlation is calculated as follows

\begin{equation}
    \label{eq:crosscorrelation}
    corr(F, F') = \frac{1}{N^2}\sum_i^N\frac{(x_i-\mu(F))({x'}_i-\mu(F'))}{\sigma(F) \sigma(F')}\text{, }
\end{equation}
where $\mu(\cdot)$ is the average value, $\sigma(\cdot)$ is the standard deviation, and $N$ is the number of values in the patterns. Correlation $corr(F, F')$ ranges in $[-1,1]$. Positive values indicates linear related series, negative inversely related series, no relationship otherwise. 

The second option, the DTW, is a robust dissimilarity measure that finds the non-linear alignment that has the lowest accumulative Euclidean distances between points, resulting in an optimal shape match preserving magnitude~\cite{keogh2005exact, muller2007dynamic}. Since the correlation is a similarity and the DTW is an unbounded dissimilarity, we transform the DTW dissimilarity into similarity to keep consistency as follows

\begin{equation}
    \label{eq:inverse}
    dtw_{sim}(F, F') = \dfrac{1}{1 + dtw(F, F')}\text{, }
\end{equation}
where $dtw(F, F')$ is the DTW distance between two patterns, and the resulting similarity $dtw_{sim}(F, F')$ ranges in $[0,1]$. 

The resulting suggestion lists contain the correlation score of all other possible variations for each of the respective nominal data, as seen in Fig.~\ref{fig:findingsuggestions}. This list represents suggestions of similar or dissimilar findings extracted from the dataset collection given the user's VQ. With these suggestion lists, users can, for instance, directly analyse other related countries or datasets of the UNData or even visualize the lists as a similarity heat-map, or, in the case of geographic information, choropleth geography maps, for example.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/suggestions.PNG}
    \caption{Example of the two suggestion lists given the dataset collection and the user's VQ (A) of the visualized time-series (B). Q4EDA calculates and outputs two suggestion lists: a dataset list indicating similar datasets to the VQ given the same time-range and categorical descriptor, and another list indicating similar categorical descriptors (e.g. country) to the VQ given the same time-range and dataset.}
    \label{fig:findingsuggestions}%TODO move the letters to the figure and remove from the caption
\end{figure}

==> paper/4_results.tex <==
\section{Use-cases and Results}
\label{sec:results}

\subsection{UNData Line charts and Wikipedia}
\label{sec:usagelinechart}

This section presents a hypothetical usage scenario of Q4EDA, showing how it can assist external VA tool users in understanding patterns of interest and building up extra knowledge during exploratory data analysis. Here we use a replica of Gapminder's line chart visualization~\cite{gapminderusaleviz} to explore the UNData dataset~\cite{undata} as a VA tool couple with an Elasticsearch~\cite{elasticsearchwikipedia} SE loaded with Wikipedia text documents~\cite{cirrussearch}. 

We introduce Justin, our fictional American High School student. He wants to investigate how the average lifespan has changed over the years in the United States. With that in mind, he visualizes the ``Life Expectancy'' indicator of the ``United States'' country (Fig.~\ref{fig:usalifeexpectancyline}). The resulting line-chart shows a positive trend toward increasing the overall American lifespan over the years. However, he notices two interesting patterns, one valley between $1860$ and $1866$ and another between $1917$ and $1919$ with some instability between $1901$ and $1930$. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/usalifeexpectancy.png}
    \caption{Life expectancy line chart of the United States. Two noticeable valleys are observed between $1860$ and $1866$ and between $1917$ and $1919$. The gray area represents the user selection.}
    \label{fig:usalifeexpectancyline}
\end{figure}

To further inspect these patterns and understand what is happening, Justin first selects the left-most valley (between $1860$ and $1866$). Internally, the enhanced VA tool uses Q4EDA to generate a search query, retrieves related Wikipedia documents, and gets a list of suggestions of related countries and datasets considering the selection (Sec.~\ref{sec:correlation}). Based on that, Justin adds the two top-ranked suggested countries to the line chart (Sweden and the United Kingdom) and realizes that the drop in life expectancy is probably an American effect since even the most related countries do not present similar valley in the same period (omitted due to space constraints). With that in mind, Justin checks the retrieved documents and observes the prevalence of the terms ``civil war'' in the returned snippets (Fig.~\ref{fig:usalifeexpectancydocs1}) and concludes that the lower life expectancy rating may result from a civil war. By reading some of the retrieved documents, he learns that the trigger of the civil war was the result of Abraham Lincoln's election and the United States southern states feeling unrepresented and/or challenged due to slavery, being able to discover one important piece for the storytelling of the United States lifespan variations, including its trigger.

Justin follows up to investigate the second dip in life expectancy and selects the period between $1917$ and $1919$. The retrieved documents' contents are, however, less homogeneous with different causes for the drop, with a span of documents discussing different topics (Fig.~\ref{fig:usalifeexpectancydocs2}). As in the previous example, he adds other top-ranked suggested countries to the line chart, including countries from different continents. Differently from the previous valley, all the included countries present a similar drop in life expectancy in the same period (Fig.~\ref{fig:usalifeexpectancylineothersef}), apparently suggesting that a global event took place. Rechecking the retrieved documents, he infers that some potential reasons for the changes in life expectancy may be the World War I and the Spanish Flu, also called Influenza Pandemic. 

%%%%
\begin{figure}[h]
    \centering
    \subfigure[Selection between $1860$ and $1866$.] {\includegraphics[width=0.48\linewidth]{figures/wikiusaearly.PNG}\label{fig:usalifeexpectancydocs1}}\quad
    %%
    \subfigure[Selection between $1917$ and $1919$.] {\includegraphics[width=0.48\linewidth]{figures/wikiusalate.PNG}\label{fig:usalifeexpectancydocs2}}
    \caption{List of documents retrieved from Wikipedia related to the drop in the United States life expectancy.}
    \label{fig:usalifeexpectancydocs}
\end{figure}
%%%%

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/usalifeexpectancyandfriends.PNG}
    \caption{Life expectancy line chart multiple countries. All countries present the same valley between $1917$ and $1919$, indicating a global reason for the drop in life expectancy.}
    \label{fig:usalifeexpectancylineothersef}
\end{figure}

Still using the countries suggestion list, Justin discovers that Russia is amongst the lowest-ranked countries and decides to investigate -- here we are discussing the country suggestion as a ranked list. Adding Russia to the line chart, Justin finds out that the reason for the similarity score being low in this period is that Russia's valley is much wider than the United States (image omitted due to space constraints). 
%
By selecting the valley in Russia's life expectancy and checking the suggested countries, he discovers that Belarus, Ukraine, Turkmenistan, Uzbekistan, Tajikistan, Kazakhstan, and Uzbekistan are the most similar to Russia. Also, by checking the retrieved documents (Fig.~\ref{fig:ursslifeexpectancydocs}), Justin discovers that during $1917$ and $1919$, Russia was facing the abolition of its monarchy in $1917$, a civil war, and the beginning of the Soviet Union, besides likely facing World War I and the Influenza Pandemic as he saw with the rest of the world.


%%%%
\begin{figure}[h]
    \centering
    \subfigure[Selection of the valley of Russia's life expectancy.] {\includegraphics[width=0.48\linewidth]{figures/russiawiki.PNG}\label{fig:ursslifeexpectancydocs}}\quad
    %%
    \subfigure[Selection of the drop of Russia's democracy index score.] {\includegraphics[width=0.48\linewidth]{figures/russiawiki2.PNG}\label{fig:ursslifeexpectancydemocracydocs}}
    \caption{List of documents retrieved from Wikipedia related to the pattern in the Russia's dataset between $1917$ and $1919$, indicating several potential events that may have affected it.}
    \label{fig:ursswiki}
\end{figure}
%%%%

Besides suggesting countries, Q4EDA also suggests other datasets with correlations given a selection (Sec.~\ref{sec:CSP}). Justin notices that the ``Democracy Index" dataset is suggested, so he creates a line-chart displaying Russia's life expectancy and democracy index together (Fig.~\ref{fig:ursslifeexpectancydemocracy}). In the resulting visual representation, he notices an inverted pattern (a valley in the life expectancy and a peak in the democracy index) between $1917$ and $1923$. Justin then selects such time period and, considering the list of returned Wikipedia documents (Fig.~\ref{fig:ursslifeexpectancydemocracydocs}), he discovers that the sudden change in the democracy index of Russia can be attributed in some part to Russia's constitution of $1918$, ``Russian Famine'', ``Russia's Civil War'' and the ``Russian Revolution", which tells about how the monarchy was abolished in $1917$ and the Soviet Union was established in $1923$, matching the steep fall of Russia's democracy index in $1923$. Justin concludes that the political landscape variation in Russia definitively impacted the lives of the Russian population, including their life expectancy.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/russiademocracy.PNG}
    \caption{Russia life expectancy and democracy index presents interesting similarities.}
    \label{fig:ursslifeexpectancydemocracy}
\end{figure}

Although an elementary analysis, Justin discovered pieces for the life-expectancy variations in the United States, including its trigger. Two different global situations, World War I and the Spanish Flu. Why Russia was differently affected than the rest of the world at the time, and much of Russia's history on revolutions and economic crisis.


\subsection{Inner Query Stability Evaluation}
\label{sec:querystability}

Although so far we assumed precise visual queries within our examples, user selection are expected to not be exact every time due to the inherent limitations of visual interfaces and means of visual selection. Therefore, we measure how much the Wikipedia results change when slight variations of VQ occur in order to evaluate \textit{R1.b} (see Sec.~\ref{sec:design}). For this, we follow \citet{Memon2004WhatTesting} and create an oracle that emulates the user behavior, allowing us to test this aspect of Q4EDA exhaustively. Notice that in this evaluation, we are not validating the search results themselves since we could not find a labeled dataset that would allow us to evaluate the connection between time-series visual patterns and the text documents of a search engine like Elasticsearch.

The oracle implementation we use is straightforward. Given a time series, we iterate over it, automatically extracting the top patterns classified by the height of their valleys and peaks; then, we vary a window around each of the patterns to generate similar selections that emulate users' selection inaccuracies. In our experiments, the window size is set to $3$, resulting in $9$ queries per pattern (one original and eight derived). This value was defined by running a test with our lab members asking them to manually select patterns in several different time series, considering the average variation among them to set the window. The stability of our query process is then measured by comparing the intersection of the set of documents retrieved using the original query $q$ and the sets of documents fetched using the derived queries $q'$. Given $D$ the set documents retrieved using the original query $q$ and $D_i$ the list of documents returned using one of the derived queries $q'_i$, the stability is computed as

\begin{equation}
\frac{1}{|D| \cdot |\Delta|} \sum_{D_i \in \Delta} |(D \cap D_i)|\text{, }
\end{equation}
where $\Delta$ is the set containing the lists of documents produced by all derived queries $q'$. Notice that the number of documents in $D$ and $D_i$ is the same and defined by the number of documents we display in our interface. In our tests, we set it to $10$.

To execute a comprehensive test, we select $960$ time series from the UNData dataset~\cite{undata} and measure the query stability for each one. We automatically detected $5,286$ relevant patterns, resulting in $47,574$ queries submitted to the search engine. Fig.~\ref{fig:querystability} summarizes the results. Overall, on average, the stability is $0.5121$, meaning that slight variations in the selection return $51\%$ of the documents returned by the original query. More specifically, peaks and valleys are more stable, with an average of around $64\%$ and a standard deviation of $0.22$. At the same time, 'unstable patterns' have less document stability with an average of $39\%$ and a standard deviation of $0.27$. This suggests that the peaks and valleys are meaningful within Q4EDA, indicating that it appropriately translates well-defined visual patterns into coherent groups of documents. Although this cannot quantify the quality of the retrieved documents, it indicates that users with similar behavior are expected to receive similar documents when attempting to select the same pattern, indicating a good degree of stability and reproducibility.

\begin{figure}[h]
    \centering
    \includegraphics[width=.75\columnwidth]{figures/violin2.eps}
    \caption{Query stability analysis. On average, slight variations in the selection return $39\%$ to $64\%$ of the documents returned by the original query depending on the pattern type, indicating a good degree of stability and reproducibility, especially for patterns with peaks and valleys.}
    \label{fig:querystability}
\end{figure}

==> paper/5_userevaluation.tex <==
\section{User Evaluation}
\label{sec:usereval}

Using the same workflow as Justin's usage scenario (see Sec.~\ref{sec:usagelinechart}), we conducted a user study to evaluate: (1) whether Q4EDA conversion method allows users to more accurately find textual information related to a specific time series pattern if compared to manually searching (\textit{R1} and \textit{R2.a}); and (2) whether users are more accurate in their query results using Q4EDA even when confident in their findings (\textit{R1.a}). We use a replica of Gapminder~\cite{rosling2012gapminderorg, gapminderusaleviz} line-chart to represent the times-series and the Wikipedia search engine. We use this setup given the Gapminder popularity and to avoid search results variations that may occur between different user profiles if, for instance, the Google search engine is employed. Through this study, we aim to check the following null hypotheses: 

\begin{quote}
$\mathbf{H^P_0}$: There is no difference in the amount of correct information related to a given pattern of interest a user can find using the proposed visual query conversion and manually querying the target search engine.
\end{quote}

\begin{quote}
$\mathbf{H^C_0}$: There is no difference in the amount of correct information related to a given pattern of interest a user who was \textbf{confident} in their answer can find using the proposed visual query conversion and manually querying the target search engine.

\end{quote}

We recruited $21$ participants of ages $16$ and up. All but two are from computer sciences, one is from social sciences, and the other claim to not have a primary area of study. Due to COVID-19, we were not able to conduct an in-person study. Instead, we conducted it through a self-guided online survey. Our experiment first conducts a demographic questionnaire and introduces the Gapminder replica with a video tutorial. Participants are then guided through an interactive tutorial using the system and finally are given a list of tasks to be performed. The study was executed in an automated and non-obstructive manner through an online survey system. Participants joined the study through their machines and had unrestricted time to complete it. The study took on average $50$ minutes, but due to the self-guided nature of online surveys, a third of the participants did not complete the study in one continuous session. 

To evaluate our hypotheses, we randomly split our participants into two groups, one containing $11$ participants, which we call \textit{Cohort 1} (\textit{C1}), and another containing $10$ participants, which we call \textit{Cohort 2} (\textit{C2}). Both groups execute two sets of tasks. For the first task, \textit{C2} is the experimental group while executing tasks using Q4EDA, and \textit{C1} is the control group executing tasks without visual queries but instead manually searching Wikipedia to find related information to the observed patterns. Therefore no search query conversion capabilities are provided to \textit{C1} as opposed to \textit{C2}. For the second task, the roles of \textit{C1} and \textit{C2} are swapped.

The benchmark of this user study was done by manually searching both Wikipedia and through visual query for the expected text documents and phrases and confirming that all tasks can be done with both tools. It is important to note that both tools use and provide interfaces to the same time-series dataset and the same textual dataset. The study does not attempt to capture all possible historical events and facts related to a pattern but only to capture some equally available to be queried in both formats.

For the first set of tasks, using the ``United States life expectancy'' dataset, we asked participants to search for probable causes for the drop between $1860$ and $1866$. We presented $5$ alternatives and asked which one is related to the observed patterns (four correct and one incorrect). Answers from the experimental group using Q4EAD were better in finding more texts related to the time-series pattern. On average, participants manually searching Wikipedia (\textit{C1}) answered correctly $31\%$ of the alternatives presented regarding related causes against $48\%$ using Q4EDA (\textit{C2}). For this task, all participants but one from \textit{C2} said they now understand better Q4EDA's usefulness for this kind of task and, by using the Q4EDA's suggestions (see Sec.~\ref{sec:correlation} and \textit{R2.b}), $7$ participants from the experimental group were also able to find other related indicators that may further enhance the exploratory analysis. 

In the second task, we swapped the two groups so that \textit{C1} is the experimental group using Q4EDA's query conversion and suggestions and \textit{C2} is the control group directly querying Wikipedia. In this task, we ask users to investigate another drop in the United States life expectancy between $1916$ and $1919$. Similar to the previous set of tasks, participants using Q4EDA had overall higher performance. Participants manually searching Wikipedia (\textit{C2}) answered correctly $38\%$ of the alternatives presented of related causes against $68\%$ using Q4EDA (\textit{C1}).

To verify our null hypothesis $\mathbf{H^P_0}$ across the two sets of tasks, we compared the control group directly using only Wikipedia and the experimental group using Q4EDA across \textbf{all} tasks. The calculated $p$-value is $P_v^{H_0}=0.0006 < 0.05$ and t-value is $T_v^{H^P_0}=-4.33$. Therefore we can confidently reject $\mathbf{H^P_0}$ and affirm that the experimental group was statistically better in finding textual information related to a pattern of interest when compared to the control group. In more specific terms, when comparing the number of answers from each group which matched our expected answers, the control group had, on average, identified $4.33$ fewer pieces of information matching our expectations than the experimental group. 

We also asked participants how confident they were with their answers to our tests. We first collected the answers where the participant was at least $Conf\geq\textit{Agree}$ in their confidence level. The resulting $p$-value is $P_v=0.011 < 0.05$, therefore rejecting the hypothesis $H^C_0$, indicating that among the participants who claim are confident in their answers, the control group has fewer answers matching what was expected when compared to similarly confident participants from the experimental group. When considering that these two groups were similarly confident in their answers, we conclude that the confidence of the control group does correlate to a correct answer as well as experimental group, or in other words, given a pattern of interest, confident Q4EDA users have more accurate textual findings than users who directly queried Wikipedia.

% To validate our analysis, we verified whether the two sets of tests or the two cohorts show significant unbalance. For this, the use as a null hypothesis: ``the two sets of tasks do not show significant difference even though they were part of the analysis of different time-frames''. The result was $P^T_v=0.0005 < 0.05$, so it can be rejected. 
% %
% We also tested the following null hypothesis: ``the two cohorts do not show significant difference''. The result was $P^C_v=0.157 > 0.05$, so again it cannot be rejected. 
% %
% Although $P^C_v$ is above close to the threshold, even when we split all our analysis by the two cohorts, most conclusions remain the same: 
% %$P^T_v(C_1)=0.05 \approx 0.05$,  $P^T_v(C_2)=0.0004 < 0.05$, 
% $P^C_v(C_1)=0.000003 < 0.05$ and $P^C_v(C_2)=0.818 > 0.05$. Since the only significant aspect which cannot be rejected is the null hypothesis of the second cohort only when analysed by itself, we can fairly confidently say that the differences between the cohorts and set of tasks were overall in agreement with our original conclusion.

In conclusion, participants of the experimental group significantly outperformed participants of the control group, showing that Q4EDA is effective in providing means for users to better and more correctly discover information in regards to a visual pattern and also to provide an effective way to convert a visual query into useful Wikipedia queries when compared to constructing the query manually. 


%
%FVP.: precisa verificar se vale a pena ficar
%
% \subsection{Historian (Expert) Interview}

% In order to evaluate Q4EDA's impact in real visualization-based data analysis applications, we interviewed Catherine, an MA student in History, while using the replica of Gapminder's line-chart from Sec.~\ref{sec:usagelinechart} to validate and align our goal with real use-cases. For her undergraduate honors thesis, Catherine researched the Second World War's effects on specific aspects of her city, omitted for confidentiality reasons. In her thesis, her research workflow involves querying open portals, such as Google and Wikipedia, through keywords about the research topic and visiting local libraries. Tasks, classified by her as long and time-consuming when considering the amount of time needed to retrieve information successfully.

% In this interview, we initially introduced Q4EDA and described the data contained within as ``World Demographics Indicators extracted from the United Nations repository''. Her initial reaction was of great interest. She demonstrated enthusiasm by the breath of potential uses of Q4EDA once she saw it working. After being shown Q4EDA's query conversion mechanism in action to retrieve relevant Wikipedia documents related to a finding of interest, Catherine explained that this simple action of visual interaction is great to empower lay users to find potential explanations for their findings. She also described that it would be of great help within her research if Q4EDA supported regional time-series data, such as provincial or municipal level, and regional text data, such as local libraries and news data, potentially reducing the effort involved in the preliminary information retrieval phase of her research. Catherine was asked how she would use Q4EDA, and she displayed significant interest in analyzing the History of Russia due to its very eventful History over the past $100$ years. Finally, she concluded our interview by saying: ``Overall, I think this is great! It is a really cool program, and I am sure a lot of people will really benefit from using it.''

==> paper/6_discussion.tex <==
\section{Discussions and Limitations}
\label{sec:limitations}

%Other domains
This paper has explored a method to convert a visual selection query into a search query usable within search engines. We tested this technique by converting patterns within world indicator dataset collections and enhancing users' analysis through Wikipedia documents. Indeed, our system is open and easily usable in other domains, which may also benefit from interpreting time-series visual selections as search queries. \obs{Different input datasets, such as news, stock market, financial data, IoT sensor data, social media, and natural disasters dataset collections could also be used in a similar fashion.} Although some of such dataset collections may be directly supported by the processes implemented so far, others may contain new data-types, which would also require new conversion processes to be implemented, requiring modification to Q4EDA's structure. We leave as future work the application of Q4EDA to other domains.

%FVP.: acho que a gente nao precisa mais falar nisso
%Alternatively, in line with our expert interview, a more fine-grained demographics analysis, considering cities or neighborhood levels and local newspaper press datasets could be supported as well, among many other potential usages. That said, the main challenge in all examples is mostly designing good visual metaphors for domain-specific problems and discovering the best SE and textual document collections to be used for each specific domain, all of which is external to Q4EDA's proposed framework. In any case, a fundamental observation has to be made: the textual snippets are not necessarily intended to find an exact cause for a particular visual finding since spurious correlations may happen. 

%results usefulness
Since we implemented Q4EDA's basic functionality, most of the exploratory tests we executed resulted in valuable retrieved textual information. However, it failed to bring meaningful documents for some specific demography indicators during our tests, though manually searching the same search engine gave similar poor results. Indeed, the usefulness of the query conversion depends on whether the SE has relevant information about the selected patterns and how well both the user and the SE can parse the data. For instance, if Wikipedia has no information on some subject for a given pattern, our framework may still return documents that may aggregate next to nothing for the analysis, which is not surprising. We forgo how to match other time-series datasets to potential SEs, expecting instead this to be decided by whoever sets up and uses our framework (e.g., external VA tools).

%FVP.: acho que a gente nao precisa mais falar nisso
%This limitation is equivalent to those presented while manually searching for information from Wikipedia, Google or any other general-purpose web search engine, such as Bing or DuckDuckGo, and was also pointed out by one of our user evaluation participants. The potential of implementing and validating output modules for domain-specific SEs certainly opens up many future works, such as evaluating the informative quality and measuring similarity between two distinct heterogeneous datasets of the same domain (e.g. medical diagnosis~\cite{zeng2012synonym}). For example, a research could be conducted to analyse the quantitative difference of information stored within text datasets, such as Wikipedia, when compared to a time-series dataset, such as the World Demographics indicator datasets by using Q4EDA. This also shows that the user is who has the actual decision and interpretative power of any of Q4EDA's output. Of course, this is due to the exploratory nature of EDA, since non-exploratory analysis, such as confirmatory analysis, would need other methods of confirming user's findings and hypothesis and consequently require to statistically prove the validity of a given search query conversion, which is another exciting and challenging future work.

Another limitation pertains to the suggestion approaches. Q4EDA suggests relevant nominal data given the visual query and the text documents by counting the number of the textual elements shared among the two either directly or through NLP. Updates to the suggestion processes are planned so that Q4EDA can also include the temporal descriptor (e.g., year) within the search or include semantic analysis over the text. The suggestion and keyword conversion processes could also benefit from other NLP techniques. Important to note that we tested other NLP techniques as part of our development process, namely Latent Dirichlet Allocation (LDA)~\cite{blei2003latent}, and DistilBert~\cite{reimers-2019-sentence-bert}. We, however, landed on the ones presented due to their speed in processing hundreds of text documents in less than a minute.

%
%FVP.: test com o google
\obs{We also tested our usage scenario and user evaluation using Google as a search engine, and the preliminary results were arguably more informative than Wikipedia.} Indeed, Google API was our first choice for most of our examples. However, its connection to the Gapminder replica was not ideal due to Google's imposed limitations, such as the limited number of API calls and limited information parsing. Also, other challenges were encountered, such as the processing of unstructured web pages as opposed to well-defined Wikipedia documents and the significant variations of results given the user's profile. %FVP.: acho que isso nao precisa mais ser dito
%Moreover, despite Wikipedia issues in terms of biased content~\cite{callahan2011cultural}, its documents are, for the good or the bad, reviewed and validated using a crowd-sourcing strategy. Most of the Internet content returned by Google is not ``verified'', with a wide range of unreliable information. 
Therefore, even though both output modules were available, we opted for Wikipedia for our examples and user evaluation. \obs{We also observed this issue when considering our evaluation process. Seen that there is no labeled dataset where patterns within time-series data are linked to textual information within a search engine, Q4EDA was unable to use common metrics, such as accuracy or f1-score, to evaluate its resulting query. However, we hope Q4EDA will instigate such labeled dataset to be compiled in the future.}
%, even though it is less comprehensive than Google.

%
%FVP.: other visual metaphors
%
\obs{Finally, although our main usage scenario focuses on a line-chart view, Q4EDA does not impose such requirements on the visual metaphor. For instance, if the Gapminder's bubble chart~\cite{gapminderbubbleviz} is used, a VQ over it would consider the two datasets displayed as the chart's axis.} Hypothetically, such a VA tool could expect a box selection within the main bubble chart visualization, which would make the VQ include one year and a range of countries. However, the VA tool could also expect a selection within the animation timeline of the bubble chart, which would make the VQ include a range of years and all available countries or even a combination of the two selection modes. In summary, Q4EDA is agnostic in terms of which visual representation was chosen.
% In summary, the visual representation is used to define a selection of a time frame in one or multiple time series. Q4EDA is agnostic in terms of visual representation.








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EXTRA INFO.. USE?
% discuss the following: when we select two metadata where patterns are opposed (going up for one and going down for the other), the query will contain both effect query terms for going up and down simultaneously. Future work could resolve this issue by preprocessing the textual database into a semantic graph format to split its meaning by the combination of patternxmetadata

% discuss: why not include more terms in the factorization of multiple combinations. It would include too many terms, which showed degenerated results

% discuss potential applications to scatterplot where patterns is not a. continuous pattren over time, but actually a pattern over the visual information of the metadata being shown in the scatterplot (say high life expectancy and low income of a selected country(ies))

% To generate the document summary, however, we use Gensim's TextRank algorithm. Other methods were attempted, such as using Bart~\cite{wolf2019huggingface}, T5~\cite{wolf2019huggingface} or Latent Dirichlet Allocation (LDA)~\cite{blei2003latent}, but due to the time required for summary generation from these other approaches, we decided to use a fast and responsive method. The summary is then displayed as plain text with the terms used in the query in bold. Moreover, a map highlighting other countries mentioned in the document and a list of related datasets are displayed (see Sec.~\ref{sec:doc2timeseries}). Sec.~\ref{fig:teaser}(F) presents an example of the detailed view of a selected document. % beyond the paper, but there is text summary as well
%  From our experiments, this form of calculating similarity performed better when utilizing LDA as opposed to other NLP methods, such as DistilBert, which is likely due to the usage of the Wikipedia corpus within LDA. % speed and wikipedia
% Although we tested with other possibilities, the LDA gave the best preliminary results in our evaluation process.
%From our experiments, this form of calculating similarity performed better when the NLTP processor utilized LDA as opposed to other NLP methods likely due to the usage of the Wikipedia corpus within LDA. 


% \subsection{Other Visual Metaphors, Datasets and Outputs}
% \label{sec:resultothers}
% Although our main usage scenario described above focuses on a line-chart view of UNData datasets~\cite{undata}, Q4EDA does not impose such requirements on the visual-metaphor nor on the dataset collection. For instance, if Justin were to use Gapminder's bubble chart instead~\cite{gapminderbubbleviz}, a VQ over the bubble chart would be comprised of the two datasets displayed as the chart's axis. Hypothetically, such VA tool could expect a box-selection within the main bubble-chart visualization, which would make the VQ include one year and a range of countries. However, the VA tool could also expect a selection within the animation timeline of the bubble-chart, which would make the VQ include a range of years and all available countries, or even a combination of the two selection modes. With this, Q4EDA's conversion and suggestion processes would output a query which follows these specifications. For instance, if one year and two datasets are within the selection, there would not be any year conversion, but the two dataset names would be given as keyword conversions. The suggestion processes would similarly follow such restrictions.

% Other datasets can also be used with Q4EDA. If instead of the UNData, a stock-market dataset~\cite{stockdataset} were to be used to display a line-chart of many individual stocks, then Q4EDA's conversion could use the stocks owner name as dataset name and the stock's country of origin. Finally, Q4EDA also could provide other output formatters, such as for google queries, or load other text documents into Elasticsearch, such as with social media dataset collections. Indeed, preliminary tests with google search also showed interesting results by performing the following changes to the final output query:

% \begin{table}[ht]
% \centering
% \begin{tabular}{lll}
% \toprule
% bnf & inner grammar & google equivalent \\ \hline
% weight-factor & superscript & order of terms \\
% negative-factor & $-$ & N/A \\
% and & $\&$ & AND \\
% or & $|$ & OR \\
% %   &  & \\ \hline
% \bottomrule
% \end{tabular}
% \end{table}

% Also, if one were to use other elasticsearch databases, such as server log files, the same Elasticsearch-based output module could hypothetically be used to query the information selected from a line-chart of, say, server events and metrics. Of course, a new output formatter could be also be implemented in order to target other SEs, such as SQL databases and Apache Lucene. These examples shows that Q4EDA is not limited to Elasticsearch and Gapminder, but due to space constraints and limitations on the underlying technologies of other SEs, such google search's as API throttle, limited website availability and different results per user profile, we focused our explanations on one application.

==> paper/7_conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, we present Q4EDA, a framework that converts a \textit{visual selection query} into a \textit{search query} format to be used in existing \textit{search engines} and, from its result, suggests other potential aspects of the data to be analysed, all of which providing a novel strategy to utilize user input for textual information retrieval.
%
The usefulness of Q4EDA is brought by an application linking a Gapminder's line-chart replica with Wikipedia documents to support exploratory analysis of world indicators. The improvement in users' exploratory analysis capability is then confirmed through a user test showing that users can find more information using Q4EDA compared to the standard manual keyword-based queries, specially when confident in their findings. The stability of the conversion process given slight variations of its inputs was also evaluated to in order to verify the applicability of Q4EDA with inaccurate visual selection interfaces.
%
Despite its limitations, Q4EDA is unique in its proposal, representing an advance toward providing solutions for querying textual information from general purpose search engines based on user interaction with visual representations.


==> paper/main.tex <==
\input{paper/1\_intro}
\input{paper/2\_related}
\input{paper/3\_method}
\input{paper/4\_results}
\input{paper/5\_userevaluation}
\input{paper/6\_discussion}
\input{paper/7\_conclusions}

% \section*{Acknowledgments}
% We acknowledge the support of the Natural Sciences and Engineering Research Council of Canada (NSERC).



% \section*{Supplementary Material}

